Semiparametric causal mediation analysis in cluster-randomized trials with post-treatment confounding

Causal mediation analysis of cluster-randomized trials can reveal how interventions affect outcomes through individual and spillover pathways. Most existing methods target natural mediation effects under assumptions that exclude treatment-induced mediator--outcome confounding. We develop a semiparametric framework for interventional mediation effects that accommodates such confounding and within-cluster interference without requiring cross-world independence assumptions. We identify cluster-average and individual-average direct and indirect effects and decompose the indirect effect into individual and spillover components, distinguishing pathways through an individual's own mediator and those of other cluster members. These contrasts evaluate hypothetical interventions on the joint mediator distribution and can differ from treatment effects carried through individual causal pathways represented by natural effects, thereby providing an intervention-oriented perspective that complements natural effects. We derive efficient influence functions to construct estimators using cluster-level cross-fitting, characterize their multiple-robustness properties, and establish conditions for asymptotic normality and semiparametric efficiency. To facilitate implementation, we develop a lower-dimensional reparameterization that reduces the need for multivariate density estimation and integration and allows nuisance functions to be estimated using parametric models or machine learning. Simulation studies evaluate finite-sample performance, and an application to a cluster-randomized trial of cognitive behavioral therapy for chronic pain illustrates the proposed methods.

==> final_results/report/simulation_tables_cluster.tex <==
% Generated from final_results(0828)/annals_simulation_bundle.rds.
% Each numerical cell is bias/RMSE/coverage/mean-SE-to-empirical-SD.
% P/AL/CI separately records point consistency, asymptotic linearity,
% and confidence-interval validity under the stated theoretical limit.

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Canonical-study performance for the IDE, $W_i=1$.}\label{tab:sim-can-IDE-C}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
C-1111 & Can-par & 1/1/1 & .004/.268/.942/.993 & .008/.211/.949/.997 & .006/.178/.955/1.012 & .002/.143/.951/1.008 \\
C-1111 & Can-SL & 1/1/1 & .001/.281/.954/1.148 & .007/.221/.959/1.046 & .006/.184/.955/1.057 & .002/.146/.955/1.034 \\
C-1111 & g-comp & 1/1/1 & .002/.236/.952/1.213 & .005/.192/.948/1.011 & .005/.162/.948/1.019 & .002/.130/.943/1.013 \\
\addlinespace[1.2pt]
C-1110 & Can-par & 1/0/0 & .001/.291/.983/1.347 & .005/.235/.986/1.393 & .005/.200/.991/1.451 & .003/.163/.993/1.513 \\
C-1110 & Can-SL & 1/0/0 & -.001/.298/.975/1.324 & .005/.239/.984/1.364 & .005/.202/.989/1.425 & .003/.164/.994/1.491 \\
C-1110 & g-comp & 1/1/1 & .002/.236/.952/1.213 & .005/.192/.948/1.011 & .005/.162/.948/1.019 & .002/.130/.943/1.013 \\
\addlinespace[1.2pt]
C-1101 & Can-par & 1/0/0 & .001/.301/.932/.961 & .011/.237/.928/.937 & .010/.207/.929/.923 & .005/.166/.928/.914 \\
C-1101 & Can-SL & 1/0/0 & .008/.310/.944/1.207 & .017/.246/.947/1.054 & .015/.212/.944/1.022 & .009/.173/.938/.966 \\
C-1101 & g-comp & 0/0/0 & .083/.263/.943/1.210 & .088/.219/.923/1.018 & .086/.188/.914/1.031 & .085/.160/.904/1.017 \\
\addlinespace[1.2pt]
C-1100 & Can-par & 1/0/0 & -.000/.285/.954/1.042 & .007/.227/.958/1.051 & .006/.196/.961/1.075 & .007/.159/.959/1.087 \\
C-1100 & Can-SL & 1/0/0 & .007/.286/.948/1.032 & .012/.228/.952/1.038 & .010/.197/.960/1.059 & .010/.160/.960/1.070 \\
C-1100 & g-comp & 0/0/0 & .083/.263/.943/1.210 & .088/.219/.923/1.018 & .086/.188/.914/1.031 & .085/.160/.904/1.017 \\
\addlinespace[1.2pt]
C-1011 & Can-par & 1/0/0 & -.019/.554/.950/.964 & .009/.440/.954/.980 & .001/.378/.952/.976 & -.004/.300/.963/1.004 \\
C-1011 & Can-SL & 1/0/0 & -.019/.544/.962/1.034 & .010/.437/.962/1.002 & .002/.375/.959/.994 & -.003/.297/.960/1.013 \\
C-1011 & g-comp & 0/0/0 & .079/.456/.955/1.155 & .105/.380/.928/1.001 & .093/.327/.924/.988 & .100/.264/.930/1.021 \\
\addlinespace[1.2pt]
C-1010 & Can-par & 1/0/0 & -.021/.562/.969/1.087 & .006/.451/.979/1.111 & .000/.388/.975/1.123 & -.003/.311/.980/1.166 \\
C-1010 & Can-SL & 1/0/0 & -.021/.548/.968/1.113 & .008/.444/.979/1.126 & .001/.384/.975/1.127 & -.002/.308/.979/1.169 \\
C-1010 & g-comp & 0/0/0 & .079/.456/.955/1.155 & .105/.380/.928/1.001 & .093/.327/.924/.988 & .100/.264/.930/1.021 \\
\addlinespace[1.2pt]
C-1001 & Can-par & 0/0/0 & .087/.471/.937/.964 & .110/.383/.934/.952 & .100/.332/.933/.946 & .094/.267/.933/.962 \\
C-1001 & Can-SL & 0/0/0 & .090/.473/.953/1.102 & .113/.390/.939/1.003 & .103/.335/.943/.991 & .096/.271/.939/.983 \\
C-1001 & g-comp & 0/0/0 & .065/.426/.959/1.186 & .095/.353/.931/1.011 & .086/.305/.925/.994 & .095/.247/.935/1.020 \\
\addlinespace[1.2pt]
C-1000 & Can-par & 0/0/0 & .086/.459/.947/.997 & .106/.375/.951/1.000 & .096/.325/.958/1.006 & .096/.265/.949/1.031 \\
C-1000 & Can-SL & 0/0/0 & .089/.454/.950/1.001 & .108/.374/.949/.995 & .098/.326/.953/.996 & .097/.265/.944/1.022 \\
C-1000 & g-comp & 0/0/0 & .065/.426/.959/1.186 & .095/.353/.931/1.011 & .086/.305/.925/.994 & .095/.247/.935/1.020 \\
\addlinespace[1.2pt]
C-0111 & Can-par & 1/0/0 & .006/.273/.949/.991 & .007/.215/.953/1.000 & .006/.183/.957/1.009 & .001/.148/.949/1.001 \\
C-0111 & Can-SL & 1/0/0 & .001/.288/.957/1.158 & .006/.227/.958/1.066 & .006/.192/.960/1.054 & .001/.153/.953/1.030 \\
C-0111 & g-comp & 0/0/0 & .001/.236/.943/1.050 & .001/.190/.940/1.018 & .001/.163/.936/1.010 & -.002/.131/.941/1.013 \\
\addlinespace[1.2pt]
C-0110 & Can-par & 0/0/0 & -.001/.299/.983/1.341 & .000/.239/.988/1.439 & -.001/.209/.992/1.478 & -.004/.172/.993/1.550 \\
C-0110 & Can-SL & 0/0/0 & -.008/.312/.977/1.315 & -.001/.249/.987/1.406 & -.003/.215/.991/1.450 & -.006/.176/.992/1.526 \\
C-0110 & g-comp & 0/0/0 & .001/.236/.943/1.050 & .001/.190/.940/1.018 & .001/.163/.936/1.010 & -.002/.131/.941/1.013 \\
\addlinespace[1.2pt]
C-0101 & Can-par & 0/0/0 & .007/.294/.933/.978 & .010/.237/.937/.948 & .011/.208/.934/.935 & .006/.169/.924/.929 \\
C-0101 & Can-SL & 0/0/0 & .006/.302/.954/1.256 & .011/.247/.958/1.067 & .013/.213/.943/1.033 & .008/.176/.937/.983 \\
C-0101 & g-comp & 0/0/0 & .079/.256/.928/1.045 & .082/.212/.921/1.020 & .082/.184/.914/1.025 & .081/.156/.905/1.016 \\
\addlinespace[1.2pt]
C-0100 & Can-par & 0/0/0 & .005/.283/.958/1.043 & .006/.227/.953/1.062 & .004/.198/.963/1.078 & .004/.161/.966/1.098 \\
C-0100 & Can-SL & 0/0/0 & .005/.287/.948/1.036 & .008/.228/.952/1.053 & .006/.200/.965/1.059 & .006/.162/.966/1.078 \\
C-0100 & g-comp & 0/0/0 & .079/.256/.928/1.045 & .082/.212/.921/1.020 & .082/.184/.914/1.025 & .081/.156/.905/1.016 \\
\addlinespace[1.2pt]
C-0011 & Can-par & 1/0/0 & -.017/.586/.952/.977 & .008/.474/.954/.981 & -.000/.410/.951/.977 & -.004/.326/.955/1.003 \\
C-0011 & Can-SL & 1/0/0 & -.019/.591/.967/1.041 & .010/.477/.960/1.009 & .000/.412/.957/.998 & -.003/.328/.957/1.014 \\
C-0011 & g-comp & 0/0/0 & .080/.490/.940/1.001 & .105/.409/.922/.982 & .091/.354/.921/.976 & .096/.286/.928/1.006 \\
\addlinespace[1.2pt]
C-0010 & Can-par & 0/0/0 & -.024/.597/.975/1.108 & .002/.486/.982/1.140 & -.007/.422/.976/1.155 & -.010/.339/.980/1.206 \\
C-0010 & Can-SL & 0/0/0 & -.028/.602/.974/1.113 & .003/.490/.982/1.146 & -.009/.423/.976/1.161 & -.011/.341/.979/1.208 \\
C-0010 & g-comp & 0/0/0 & .080/.490/.940/1.001 & .105/.409/.922/.982 & .091/.354/.921/.976 & .096/.286/.928/1.006 \\
\addlinespace[1.2pt]
C-0001 & Can-par & 0/0/0 & .094/.498/.954/.982 & .112/.415/.928/.953 & .100/.361/.929/.950 & .095/.295/.929/.955 \\
C-0001 & Can-SL & 0/0/0 & .095/.511/.959/1.112 & .112/.428/.937/.999 & .101/.368/.938/.989 & .096/.301/.936/.977 \\
C-0001 & g-comp & 0/0/0 & .060/.454/.943/1.013 & .091/.376/.926/.992 & .083/.329/.921/.981 & .090/.266/.927/1.008 \\
\addlinespace[1.2pt]
C-0000 & Can-par & 0/0/0 & .093/.489/.951/1.004 & .108/.408/.943/.992 & .094/.355/.954/.998 & .093/.289/.946/1.020 \\
C-0000 & Can-SL & 0/0/0 & .094/.499/.946/1.001 & .109/.415/.945/.984 & .094/.360/.949/.986 & .094/.291/.940/1.012 \\
C-0000 & g-comp & 0/0/0 & .060/.454/.943/1.013 & .091/.376/.926/.992 & .083/.329/.921/.981 & .090/.266/.927/1.008 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Canonical-study performance for the IIME, $W_i=1$.}\label{tab:sim-can-IIME-C}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
C-1111 & Can-par & 1/1/1 & -.006/.227/.963/1.009 & -.004/.187/.954/.983 & -.010/.159/.953/.995 & -.001/.126/.959/1.012 \\
C-1111 & Can-SL & 1/1/1 & -.010/.225/.960/1.000 & -.006/.186/.952/.976 & -.009/.158/.953/.991 & -.001/.126/.956/1.010 \\
C-1111 & g-comp & 1/1/1 & -.001/.176/.952/1.056 & .001/.146/.940/1.000 & .000/.126/.935/.984 & .002/.099/.941/1.013 \\
\addlinespace[1.2pt]
C-1110 & Can-par & 1/0/0 & -.006/.226/.964/1.018 & -.004/.186/.959/.993 & -.010/.159/.953/1.003 & -.001/.126/.962/1.025 \\
C-1110 & Can-SL & 1/0/0 & -.011/.224/.961/1.004 & -.006/.185/.957/.985 & -.010/.158/.954/.997 & -.002/.126/.958/1.020 \\
C-1110 & g-comp & 1/1/1 & -.001/.176/.952/1.056 & .001/.146/.940/1.000 & .000/.126/.935/.984 & .002/.099/.941/1.013 \\
\addlinespace[1.2pt]
C-1101 & Can-par & 0/0/0 & -.079/.384/.952/.974 & -.063/.312/.950/.979 & -.076/.278/.940/.965 & -.069/.226/.942/.984 \\
C-1101 & Can-SL & 0/0/0 & -.089/.376/.951/.967 & -.068/.309/.947/.974 & -.080/.276/.935/.962 & -.071/.225/.945/.985 \\
C-1101 & g-comp & 0/0/0 & -.069/.268/.934/1.044 & -.058/.229/.923/.980 & -.065/.202/.916/.976 & -.063/.163/.923/1.009 \\
\addlinespace[1.2pt]
C-1100 & Can-par & 0/0/0 & -.078/.385/.953/.977 & -.062/.313/.952/.981 & -.076/.278/.939/.967 & -.069/.226/.944/.992 \\
C-1100 & Can-SL & 0/0/0 & -.089/.378/.946/.964 & -.067/.309/.951/.974 & -.079/.276/.937/.963 & -.071/.224/.945/.991 \\
C-1100 & g-comp & 0/0/0 & -.069/.268/.934/1.044 & -.058/.229/.923/.980 & -.065/.202/.916/.976 & -.063/.163/.923/1.009 \\
\addlinespace[1.2pt]
C-1011 & Can-par & 1/0/0 & -.009/.190/.964/1.013 & -.002/.158/.956/.977 & -.006/.134/.956/.988 & -.001/.105/.959/1.013 \\
C-1011 & Can-SL & 1/0/0 & -.014/.193/.957/1.000 & -.006/.161/.951/.960 & -.007/.136/.952/.972 & -.001/.107/.953/1.003 \\
C-1011 & g-comp & 0/0/0 & -.002/.177/.953/1.064 & .002/.148/.941/1.006 & .000/.129/.935/.981 & .003/.100/.941/1.011 \\
\addlinespace[1.2pt]
C-1010 & Can-par & 1/0/0 & -.009/.189/.964/1.026 & -.002/.158/.957/.987 & -.006/.134/.957/.998 & -.001/.105/.962/1.032 \\
C-1010 & Can-SL & 1/0/0 & -.015/.191/.960/1.007 & -.006/.160/.953/.971 & -.007/.136/.951/.980 & -.002/.106/.956/1.018 \\
C-1010 & g-comp & 0/0/0 & -.002/.177/.953/1.064 & .002/.148/.941/1.006 & .000/.129/.935/.981 & .003/.100/.941/1.011 \\
\addlinespace[1.2pt]
C-1001 & Can-par & 0/0/0 & -.094/.308/.932/1.004 & -.073/.259/.925/.967 & -.080/.226/.915/.971 & -.072/.184/.911/.993 \\
C-1001 & Can-SL & 0/0/0 & -.105/.311/.924/.992 & -.079/.262/.923/.956 & -.085/.228/.909/.968 & -.074/.185/.912/.989 \\
C-1001 & g-comp & 0/0/0 & -.056/.283/.935/1.035 & -.047/.242/.925/.981 & -.058/.212/.919/.976 & -.057/.172/.925/1.006 \\
\addlinespace[1.2pt]
C-1000 & Can-par & 0/0/0 & -.093/.308/.936/1.010 & -.072/.259/.928/.970 & -.079/.227/.921/.974 & -.073/.184/.913/1.003 \\
C-1000 & Can-SL & 0/0/0 & -.105/.312/.921/.988 & -.079/.263/.924/.955 & -.085/.229/.913/.969 & -.075/.186/.910/.995 \\
C-1000 & g-comp & 0/0/0 & -.056/.283/.935/1.035 & -.047/.242/.925/.981 & -.058/.212/.919/.976 & -.057/.172/.925/1.006 \\
\addlinespace[1.2pt]
C-0111 & Can-par & 1/0/0 & -.010/.221/.962/1.005 & -.006/.183/.956/.974 & -.011/.155/.954/.988 & -.002/.124/.955/.997 \\
C-0111 & Can-SL & 1/0/0 & -.017/.221/.957/1.002 & -.011/.183/.948/.966 & -.013/.155/.950/.983 & -.004/.124/.956/.995 \\
C-0111 & g-comp & 0/0/0 & -.020/.171/.952/1.054 & -.017/.141/.935/1.001 & -.019/.123/.936/.985 & -.017/.096/.941/1.015 \\
\addlinespace[1.2pt]
C-0110 & Can-par & 0/0/0 & -.015/.220/.964/1.015 & -.012/.182/.959/.988 & -.017/.155/.952/1.001 & -.009/.123/.957/1.019 \\
C-0110 & Can-SL & 0/0/0 & -.021/.220/.959/1.005 & -.016/.182/.955/.979 & -.019/.155/.951/.993 & -.011/.123/.956/1.014 \\
C-0110 & g-comp & 0/0/0 & -.020/.171/.952/1.054 & -.017/.141/.935/1.001 & -.019/.123/.936/.985 & -.017/.096/.941/1.015 \\
\addlinespace[1.2pt]
C-0101 & Can-par & 0/0/0 & -.118/.374/.945/.984 & -.100/.307/.944/.984 & -.111/.276/.927/.972 & -.103/.229/.928/.988 \\
C-0101 & Can-SL & 0/0/0 & -.126/.370/.940/.982 & -.104/.305/.940/.984 & -.113/.275/.928/.970 & -.104/.227/.926/.990 \\
C-0101 & g-comp & 0/0/0 & -.120/.279/.918/1.038 & -.109/.242/.906/.979 & -.117/.220/.873/.977 & -.116/.187/.864/1.007 \\
\addlinespace[1.2pt]
C-0100 & Can-par & 0/0/0 & -.119/.375/.947/.987 & -.102/.308/.944/.989 & -.113/.277/.926/.975 & -.107/.230/.928/.999 \\
C-0100 & Can-SL & 0/0/0 & -.127/.371/.940/.981 & -.106/.305/.944/.985 & -.116/.276/.925/.971 & -.108/.228/.926/.997 \\
C-0100 & g-comp & 0/0/0 & -.120/.279/.918/1.038 & -.109/.242/.906/.979 & -.117/.220/.873/.977 & -.116/.187/.864/1.007 \\
\addlinespace[1.2pt]
C-0011 & Can-par & 1/0/0 & -.013/.186/.962/1.006 & -.004/.155/.953/.964 & -.006/.131/.950/.970 & -.002/.104/.954/.986 \\
C-0011 & Can-SL & 1/0/0 & -.022/.190/.958/1.004 & -.010/.159/.948/.951 & -.010/.134/.947/.958 & -.004/.105/.952/.980 \\
C-0011 & g-comp & 0/0/0 & -.021/.173/.953/1.063 & -.016/.144/.936/1.008 & -.018/.126/.926/.983 & -.016/.098/.940/1.013 \\
\addlinespace[1.2pt]
C-0010 & Can-par & 0/0/0 & -.019/.185/.963/1.019 & -.010/.154/.957/.982 & -.013/.130/.953/.990 & -.009/.102/.957/1.021 \\
C-0010 & Can-SL & 0/0/0 & -.026/.189/.956/1.009 & -.015/.158/.950/.968 & -.016/.134/.947/.974 & -.011/.104/.955/1.010 \\
C-0010 & g-comp & 0/0/0 & -.021/.173/.953/1.063 & -.016/.144/.936/1.008 & -.018/.126/.926/.983 & -.016/.098/.940/1.013 \\
\addlinespace[1.2pt]
C-0001 & Can-par & 0/0/0 & -.136/.314/.916/1.007 & -.111/.264/.907/.967 & -.115/.233/.881/.975 & -.107/.195/.875/.993 \\
C-0001 & Can-SL & 0/0/0 & -.145/.320/.913/1.005 & -.117/.269/.905/.963 & -.119/.237/.875/.974 & -.108/.196/.873/.991 \\
C-0001 & g-comp & 0/0/0 & -.105/.293/.918/1.029 & -.098/.254/.910/.980 & -.109/.228/.885/.978 & -.110/.194/.877/1.004 \\
\addlinespace[1.2pt]
C-0000 & Can-par & 0/0/0 & -.137/.314/.920/1.016 & -.113/.265/.911/.976 & -.117/.234/.886/.987 & -.110/.196/.869/1.011 \\
C-0000 & Can-SL & 0/0/0 & -.146/.321/.917/1.007 & -.119/.271/.904/.965 & -.122/.238/.883/.981 & -.112/.198/.874/1.003 \\
C-0000 & g-comp & 0/0/0 & -.105/.293/.918/1.029 & -.098/.254/.910/.980 & -.109/.228/.885/.978 & -.110/.194/.877/1.004 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Canonical-study performance for the ISME, $W_i=1$.}\label{tab:sim-can-ISME-C}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
C-1111 & Can-par & 1/1/1 & .000/.140/.922/.983 & -.002/.104/.919/.997 & .000/.088/.930/.989 & .002/.067/.940/1.005 \\
C-1111 & Can-SL & 1/1/1 & -.002/.147/.926/1.108 & -.000/.108/.929/1.063 & .001/.092/.933/1.036 & .003/.069/.948/1.048 \\
C-1111 & g-comp & 1/1/1 & -.002/.114/.952/1.254 & -.003/.089/.936/1.057 & -.001/.078/.927/.999 & .000/.060/.946/1.031 \\
\addlinespace[1.2pt]
C-1110 & Can-par & 1/0/0 & .002/.138/.948/1.165 & -.003/.104/.959/1.233 & .001/.089/.958/1.208 & .002/.069/.977/1.281 \\
C-1110 & Can-SL & 1/0/0 & .001/.143/.946/1.188 & -.002/.106/.959/1.238 & .002/.092/.964/1.216 & .002/.070/.975/1.301 \\
C-1110 & g-comp & 1/1/1 & -.002/.114/.952/1.254 & -.003/.089/.936/1.057 & -.001/.078/.927/.999 & .000/.060/.946/1.031 \\
\addlinespace[1.2pt]
C-1101 & Can-par & 0/0/0 & .064/.185/.934/.904 & .064/.148/.926/.919 & .062/.133/.910/.887 & .064/.111/.902/.927 \\
C-1101 & Can-SL & 0/0/0 & .063/.183/.939/.966 & .064/.147/.935/.953 & .060/.132/.920/.907 & .063/.111/.907/.945 \\
C-1101 & g-comp & 0/0/0 & .060/.171/.963/1.185 & .063/.141/.938/1.048 & .058/.124/.926/1.007 & .063/.107/.897/1.015 \\
\addlinespace[1.2pt]
C-1100 & Can-par & 0/0/0 & .064/.187/.942/.928 & .064/.147/.945/.968 & .061/.132/.936/.934 & .064/.112/.922/.980 \\
C-1100 & Can-SL & 0/0/0 & .066/.186/.947/.947 & .064/.147/.943/.975 & .061/.132/.933/.930 & .064/.111/.923/.981 \\
C-1100 & g-comp & 0/0/0 & .060/.171/.963/1.185 & .063/.141/.938/1.048 & .058/.124/.926/1.007 & .063/.107/.897/1.015 \\
\addlinespace[1.2pt]
C-1011 & Can-par & 1/0/0 & .000/.140/.922/.983 & -.002/.104/.919/.997 & .000/.088/.930/.989 & .002/.067/.940/1.005 \\
C-1011 & Can-SL & 1/0/0 & -.002/.147/.927/1.107 & -.000/.108/.929/1.063 & .001/.092/.934/1.036 & .003/.069/.948/1.048 \\
C-1011 & g-comp & 0/0/0 & -.002/.114/.952/1.254 & -.003/.089/.936/1.057 & -.001/.078/.927/.999 & .000/.060/.946/1.031 \\
\addlinespace[1.2pt]
C-1010 & Can-par & 1/0/0 & .002/.138/.948/1.165 & -.003/.104/.959/1.233 & .001/.089/.958/1.208 & .002/.069/.977/1.281 \\
C-1010 & Can-SL & 1/0/0 & .001/.143/.947/1.188 & -.002/.106/.959/1.238 & .002/.092/.964/1.216 & .002/.070/.975/1.301 \\
C-1010 & g-comp & 0/0/0 & -.002/.114/.952/1.254 & -.003/.089/.936/1.057 & -.001/.078/.927/.999 & .000/.060/.946/1.031 \\
\addlinespace[1.2pt]
C-1001 & Can-par & 0/0/0 & .064/.185/.934/.904 & .064/.148/.926/.919 & .062/.133/.910/.887 & .064/.111/.902/.927 \\
C-1001 & Can-SL & 0/0/0 & .063/.183/.937/.965 & .064/.147/.936/.952 & .060/.132/.920/.906 & .063/.111/.908/.944 \\
C-1001 & g-comp & 0/0/0 & .060/.171/.963/1.185 & .063/.141/.938/1.048 & .058/.124/.926/1.007 & .063/.107/.897/1.015 \\
\addlinespace[1.2pt]
C-1000 & Can-par & 0/0/0 & .064/.187/.942/.928 & .064/.147/.945/.968 & .061/.132/.936/.934 & .064/.112/.922/.980 \\
C-1000 & Can-SL & 0/0/0 & .066/.186/.946/.946 & .064/.147/.943/.974 & .061/.132/.933/.930 & .064/.111/.921/.980 \\
C-1000 & g-comp & 0/0/0 & .060/.171/.963/1.185 & .063/.141/.938/1.048 & .058/.124/.926/1.007 & .063/.107/.897/1.015 \\
\addlinespace[1.2pt]
C-0111 & Can-par & 1/0/0 & .003/.145/.932/1.022 & .001/.109/.941/1.028 & .002/.093/.944/1.025 & .002/.071/.953/1.056 \\
C-0111 & Can-SL & 1/0/0 & .008/.152/.944/1.158 & .007/.115/.945/1.103 & .006/.097/.952/1.080 & .005/.074/.957/1.096 \\
C-0111 & g-comp & 0/0/0 & .019/.116/.954/1.092 & .019/.094/.944/1.034 & .022/.084/.928/.975 & .023/.065/.943/1.045 \\
\addlinespace[1.2pt]
C-0110 & Can-par & 0/0/0 & .013/.140/.959/1.210 & .009/.109/.970/1.261 & .012/.095/.970/1.257 & .014/.074/.986/1.347 \\
C-0110 & Can-SL & 0/0/0 & .018/.148/.962/1.224 & .015/.114/.974/1.272 & .017/.100/.975/1.264 & .018/.077/.986/1.369 \\
C-0110 & g-comp & 0/0/0 & .019/.116/.954/1.092 & .019/.094/.944/1.034 & .022/.084/.928/.975 & .023/.065/.943/1.045 \\
\addlinespace[1.2pt]
C-0101 & Can-par & 0/0/0 & .104/.203/.951/.964 & .101/.171/.923/.978 & .096/.156/.899/.939 & .097/.135/.872/1.004 \\
C-0101 & Can-SL & 0/0/0 & .107/.207/.952/1.024 & .104/.174/.932/1.002 & .096/.156/.907/.955 & .097/.135/.871/1.016 \\
C-0101 & g-comp & 0/0/0 & .115/.204/.929/1.049 & .119/.180/.882/1.018 & .115/.164/.838/.985 & .120/.151/.741/1.029 \\
\addlinespace[1.2pt]
C-0100 & Can-par & 0/0/0 & .103/.205/.958/.985 & .103/.172/.947/1.023 & .098/.158/.922/.978 & .101/.139/.884/1.049 \\
C-0100 & Can-SL & 0/0/0 & .107/.209/.957/.998 & .106/.175/.940/1.025 & .101/.160/.916/.973 & .103/.140/.879/1.045 \\
C-0100 & g-comp & 0/0/0 & .115/.204/.929/1.049 & .119/.180/.882/1.018 & .115/.164/.838/.985 & .120/.151/.741/1.029 \\
\addlinespace[1.2pt]
C-0011 & Can-par & 1/0/0 & .003/.145/.932/1.022 & .001/.109/.941/1.028 & .002/.093/.944/1.025 & .002/.071/.953/1.056 \\
C-0011 & Can-SL & 1/0/0 & .008/.153/.945/1.158 & .007/.115/.942/1.103 & .006/.097/.953/1.082 & .005/.074/.958/1.096 \\
C-0011 & g-comp & 0/0/0 & .019/.116/.954/1.092 & .019/.094/.944/1.034 & .022/.084/.928/.975 & .023/.065/.943/1.045 \\
\addlinespace[1.2pt]
C-0010 & Can-par & 0/0/0 & .013/.140/.959/1.210 & .009/.109/.970/1.261 & .012/.095/.970/1.257 & .014/.074/.986/1.347 \\
C-0010 & Can-SL & 0/0/0 & .018/.148/.963/1.225 & .015/.114/.973/1.272 & .017/.100/.975/1.265 & .018/.077/.985/1.370 \\
C-0010 & g-comp & 0/0/0 & .019/.116/.954/1.092 & .019/.094/.944/1.034 & .022/.084/.928/.975 & .023/.065/.943/1.045 \\
\addlinespace[1.2pt]
C-0001 & Can-par & 0/0/0 & .104/.203/.951/.964 & .101/.171/.923/.978 & .096/.156/.899/.939 & .097/.135/.872/1.004 \\
C-0001 & Can-SL & 0/0/0 & .107/.207/.952/1.024 & .104/.173/.932/1.002 & .096/.156/.909/.957 & .097/.135/.870/1.017 \\
C-0001 & g-comp & 0/0/0 & .115/.204/.929/1.049 & .119/.180/.882/1.018 & .115/.164/.838/.985 & .120/.151/.741/1.029 \\
\addlinespace[1.2pt]
C-0000 & Can-par & 0/0/0 & .103/.205/.958/.985 & .103/.172/.947/1.023 & .098/.158/.922/.978 & .101/.139/.884/1.049 \\
C-0000 & Can-SL & 0/0/0 & .107/.209/.958/.999 & .106/.175/.941/1.025 & .101/.160/.918/.974 & .103/.140/.879/1.045 \\
C-0000 & g-comp & 0/0/0 & .115/.204/.929/1.049 & .119/.180/.882/1.018 & .115/.164/.838/.985 & .120/.151/.741/1.029 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Low-dimensional-study performance for the IDE, $W_i=1$.}\label{tab:sim-ld-IDE-C}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
LD-AC & G+glmnet & 1/1/1 & .004/.271/.946/1.068 & .006/.213/.953/1.046 & .007/.180/.957/1.034 & .003/.144/.958/1.037 \\
LD-AC & G+RF & 1/1/1 & .003/.276/.949/1.074 & .006/.218/.952/1.045 & .006/.181/.962/1.055 & .001/.144/.952/1.043 \\
LD-AC & G+SL & 1/1/1 & -.000/.280/.970/1.346 & .006/.225/.962/1.146 & .006/.185/.963/1.106 & .002/.146/.965/1.086 \\
LD-AC & RB+glmnet & 1/1/1 & .004/.271/.945/1.067 & .006/.213/.950/1.044 & .006/.179/.959/1.040 & .003/.145/.953/1.037 \\
LD-AC & RB+RF & 1/1/1 & .003/.277/.949/1.068 & .005/.217/.953/1.051 & .006/.181/.962/1.052 & .001/.144/.958/1.043 \\
LD-AC & RB+SL & 1/1/1 & .002/.283/.965/1.329 & .004/.227/.964/1.137 & .006/.184/.968/1.113 & .003/.147/.963/1.084 \\
\addlinespace[1.2pt]
LD-T2 & G+glmnet & 1/0/0 & .003/.268/.948/1.048 & .008/.209/.952/1.018 & .006/.178/.951/1.000 & .002/.142/.950/1.002 \\
LD-T2 & G+RF & 1/0/0 & .000/.284/.951/1.090 & .003/.229/.959/1.098 & .005/.197/.972/1.127 & .002/.161/.977/1.202 \\
LD-T2 & G+SL & 1/0/0 & .000/.280/.977/1.452 & .009/.223/.988/1.629 & .003/.187/.991/1.670 & .002/.147/.985/1.406 \\
LD-T2 & RB+glmnet & 1/0/0 & .004/.267/.949/1.051 & .008/.209/.955/1.020 & .007/.178/.951/.998 & .002/.142/.955/1.003 \\
LD-T2 & RB+RF & 1/0/0 & -.001/.283/.956/1.094 & .005/.228/.967/1.100 & .007/.195/.970/1.135 & .003/.160/.984/1.206 \\
LD-T2 & RB+SL & 1/0/0 & -.002/.283/.979/1.451 & .007/.222/.988/1.638 & .006/.186/.989/1.683 & .002/.145/.985/1.427 \\
\addlinespace[1.2pt]
LD-T3 & G+glmnet & 1/0/0 & .020/.274/.949/1.083 & .017/.217/.954/1.060 & .018/.185/.958/1.044 & .013/.150/.954/1.042 \\
LD-T3 & G+RF & 1/0/0 & .019/.279/.954/1.085 & .017/.220/.961/1.068 & .017/.186/.964/1.064 & .010/.149/.955/1.049 \\
LD-T3 & G+SL & 1/0/0 & .014/.283/.965/1.351 & .015/.230/.966/1.156 & .015/.190/.965/1.128 & .009/.151/.963/1.097 \\
LD-T3 & RB+glmnet & 1/0/0 & .020/.274/.951/1.079 & .017/.218/.955/1.052 & .017/.185/.957/1.051 & .012/.150/.957/1.045 \\
LD-T3 & RB+RF & 1/0/0 & .020/.279/.953/1.083 & .016/.220/.959/1.067 & .017/.187/.964/1.059 & .011/.150/.955/1.046 \\
LD-T3 & RB+SL & 1/0/0 & .017/.284/.966/1.343 & .011/.232/.961/1.150 & .015/.189/.971/1.132 & .009/.151/.958/1.095 \\
\addlinespace[1.2pt]
LD-T4 & G+glmnet & 0/0/0 & .008/.268/.954/1.044 & .007/.210/.950/1.030 & .010/.181/.950/1.003 & .004/.147/.949/1.014 \\
LD-T4 & G+RF & 0/0/0 & .008/.273/.957/1.049 & .007/.213/.958/1.039 & .009/.183/.953/1.019 & .002/.145/.951/1.018 \\
LD-T4 & G+SL & 0/0/0 & .004/.276/.967/1.328 & .005/.224/.966/1.138 & .008/.187/.959/1.078 & .002/.147/.957/1.065 \\
LD-T4 & RB+glmnet & 0/0/0 & .009/.268/.954/1.042 & .007/.211/.949/1.023 & .009/.181/.950/1.006 & .004/.147/.952/1.017 \\
LD-T4 & RB+RF & 0/0/0 & .008/.274/.959/1.046 & .006/.213/.955/1.038 & .009/.183/.954/1.018 & .003/.146/.953/1.018 \\
LD-T4 & RB+SL & 0/0/0 & .006/.280/.973/1.314 & .002/.225/.958/1.132 & .008/.186/.966/1.085 & .002/.149/.957/1.059 \\
\addlinespace[1.2pt]
LD-T5 & G+glmnet & 0/0/0 & .019/.274/.952/1.083 & .017/.218/.957/1.055 & .016/.184/.959/1.047 & .012/.148/.954/1.031 \\
LD-T5 & G+RF & 0/0/0 & .014/.287/.954/1.134 & .011/.236/.967/1.145 & .014/.206/.975/1.161 & .013/.168/.984/1.235 \\
LD-T5 & G+SL & 0/0/0 & .014/.282/.973/1.494 & .015/.232/.986/1.667 & .014/.195/.993/1.733 & .011/.154/.986/1.469 \\
LD-T5 & RB+glmnet & 0/0/0 & .019/.273/.952/1.086 & .016/.217/.955/1.058 & .017/.185/.958/1.045 & .011/.147/.958/1.037 \\
LD-T5 & RB+RF & 0/0/0 & .014/.286/.953/1.132 & .010/.236/.966/1.141 & .017/.205/.971/1.164 & .013/.168/.982/1.235 \\
LD-T5 & RB+SL & 0/0/0 & .014/.285/.980/1.486 & .011/.230/.990/1.692 & .015/.193/.991/1.755 & .011/.153/.987/1.478 \\
\addlinespace[1.2pt]
LD-T6 & G+glmnet & 0/0/0 & .007/.269/.954/1.044 & .007/.210/.951/1.025 & .008/.180/.950/1.005 & .003/.145/.952/1.002 \\
LD-T6 & G+RF & 0/0/0 & .003/.284/.958/1.092 & .000/.231/.966/1.108 & .006/.202/.970/1.132 & .004/.165/.978/1.207 \\
LD-T6 & G+SL & 0/0/0 & .004/.280/.978/1.450 & .005/.227/.987/1.647 & .005/.191/.990/1.703 & .002/.151/.983/1.433 \\
LD-T6 & RB+glmnet & 0/0/0 & .008/.268/.954/1.048 & .006/.209/.952/1.030 & .009/.182/.950/.998 & .003/.144/.955/1.007 \\
LD-T6 & RB+RF & 0/0/0 & .003/.282/.961/1.100 & .001/.231/.965/1.106 & .008/.201/.973/1.131 & .004/.166/.978/1.204 \\
LD-T6 & RB+SL & 0/0/0 & .004/.282/.979/1.448 & .002/.224/.989/1.672 & .006/.190/.989/1.718 & .002/.150/.987/1.450 \\
\addlinespace[1.2pt]
LD-U2 & G+glmnet & 1/0/0 & .004/.271/.946/1.068 & .006/.213/.953/1.046 & .007/.180/.957/1.034 & .003/.144/.958/1.037 \\
LD-U2 & G+RF & 1/0/0 & .003/.276/.949/1.074 & .006/.218/.952/1.045 & .006/.181/.962/1.055 & .001/.144/.952/1.043 \\
LD-U2 & G+SL & 1/0/0 & -.000/.280/.970/1.346 & .006/.225/.962/1.146 & .006/.185/.963/1.106 & .002/.146/.965/1.086 \\
LD-U2 & RB+glmnet & 1/0/0 & .004/.271/.945/1.067 & .006/.213/.950/1.044 & .006/.179/.959/1.040 & .003/.145/.953/1.037 \\
LD-U2 & RB+RF & 1/0/0 & .003/.277/.949/1.068 & .005/.217/.953/1.051 & .006/.181/.962/1.052 & .001/.144/.958/1.043 \\
LD-U2 & RB+SL & 1/0/0 & .002/.283/.965/1.329 & .004/.227/.964/1.137 & .006/.184/.968/1.113 & .003/.147/.963/1.084 \\
\addlinespace[1.2pt]
LD-U3 & G+glmnet & 1/0/0 & .004/.271/.946/1.068 & .006/.213/.953/1.046 & .007/.180/.957/1.034 & .003/.144/.958/1.037 \\
LD-U3 & G+RF & 1/0/0 & .003/.276/.949/1.074 & .006/.218/.952/1.045 & .006/.181/.962/1.055 & .001/.144/.952/1.043 \\
LD-U3 & G+SL & 1/0/0 & -.000/.280/.970/1.346 & .006/.225/.962/1.146 & .006/.185/.963/1.106 & .002/.146/.965/1.086 \\
LD-U3 & RB+glmnet & 1/0/0 & .004/.271/.945/1.067 & .006/.213/.950/1.044 & .006/.179/.959/1.040 & .003/.145/.953/1.037 \\
LD-U3 & RB+RF & 1/0/0 & .003/.277/.949/1.068 & .005/.217/.953/1.051 & .006/.181/.962/1.052 & .001/.144/.958/1.043 \\
LD-U3 & RB+SL & 1/0/0 & .002/.283/.965/1.329 & .004/.227/.964/1.137 & .006/.184/.968/1.113 & .003/.147/.963/1.084 \\
\addlinespace[1.2pt]
LD-U4 & G+glmnet & 1/0/0 & .004/.271/.946/1.068 & .006/.213/.953/1.046 & .007/.180/.957/1.034 & .003/.144/.958/1.037 \\
LD-U4 & G+RF & 1/0/0 & .003/.276/.949/1.074 & .006/.218/.952/1.045 & .006/.181/.962/1.055 & .001/.144/.952/1.043 \\
LD-U4 & G+SL & 1/0/0 & -.000/.280/.970/1.346 & .006/.225/.962/1.146 & .006/.185/.963/1.106 & .002/.146/.965/1.086 \\
LD-U4 & RB+glmnet & 1/0/0 & .004/.271/.945/1.067 & .006/.213/.950/1.044 & .006/.179/.959/1.040 & .003/.145/.953/1.037 \\
LD-U4 & RB+RF & 1/0/0 & .003/.277/.949/1.068 & .005/.217/.953/1.051 & .006/.181/.962/1.052 & .001/.144/.958/1.043 \\
LD-U4 & RB+SL & 1/0/0 & .002/.283/.965/1.329 & .004/.227/.964/1.137 & .006/.184/.968/1.113 & .003/.147/.963/1.084 \\
\addlinespace[1.2pt]
LD-U5 & G+glmnet & 1/0/0 & .004/.271/.946/1.068 & .006/.213/.953/1.046 & .007/.180/.957/1.034 & .003/.144/.958/1.037 \\
LD-U5 & G+RF & 1/0/0 & .003/.276/.949/1.074 & .006/.218/.952/1.045 & .006/.181/.962/1.055 & .001/.144/.952/1.043 \\
LD-U5 & G+SL & 1/0/0 & -.000/.280/.970/1.346 & .006/.225/.962/1.146 & .006/.185/.963/1.106 & .002/.146/.965/1.086 \\
LD-U5 & RB+glmnet & 1/0/0 & .004/.271/.945/1.067 & .006/.213/.950/1.044 & .006/.179/.959/1.040 & .003/.145/.953/1.037 \\
LD-U5 & RB+RF & 1/0/0 & .003/.277/.949/1.068 & .005/.217/.953/1.051 & .006/.181/.962/1.052 & .001/.144/.958/1.043 \\
LD-U5 & RB+SL & 1/0/0 & .002/.283/.965/1.329 & .004/.227/.964/1.137 & .006/.184/.968/1.113 & .003/.147/.963/1.084 \\
\addlinespace[1.2pt]
LD-U6 & G+glmnet & 1/0/0 & .004/.271/.946/1.068 & .006/.213/.953/1.046 & .007/.180/.957/1.034 & .003/.144/.958/1.037 \\
LD-U6 & G+RF & 1/0/0 & .003/.276/.949/1.074 & .006/.218/.952/1.045 & .006/.181/.962/1.055 & .001/.144/.952/1.043 \\
LD-U6 & G+SL & 1/0/0 & -.000/.280/.970/1.346 & .006/.225/.962/1.146 & .006/.185/.963/1.106 & .002/.146/.965/1.086 \\
LD-U6 & RB+glmnet & 1/0/0 & .004/.271/.945/1.067 & .006/.213/.950/1.044 & .006/.179/.959/1.040 & .003/.145/.953/1.037 \\
LD-U6 & RB+RF & 1/0/0 & .003/.277/.949/1.068 & .005/.217/.953/1.051 & .006/.181/.962/1.052 & .001/.144/.958/1.043 \\
LD-U6 & RB+SL & 1/0/0 & .002/.283/.965/1.329 & .004/.227/.964/1.137 & .006/.184/.968/1.113 & .003/.147/.963/1.084 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Low-dimensional-study performance for the IIME, $W_i=1$.}\label{tab:sim-ld-IIME-C}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
LD-AC & G+glmnet & 1/1/1 & -.006/.233/.963/1.073 & -.003/.189/.961/1.007 & -.008/.160/.953/1.004 & -.000/.127/.958/1.017 \\
LD-AC & G+RF & 1/1/1 & -.006/.232/.966/1.073 & -.004/.189/.962/1.006 & -.008/.160/.956/1.004 & -.001/.126/.957/1.018 \\
LD-AC & G+SL & 1/1/1 & -.006/.231/.968/1.083 & -.003/.189/.961/1.011 & -.008/.160/.955/1.007 & -.001/.126/.958/1.021 \\
LD-AC & RB+glmnet & 1/1/1 & -.006/.233/.964/1.073 & -.004/.189/.961/1.006 & -.008/.160/.953/1.004 & -.001/.126/.960/1.019 \\
LD-AC & RB+RF & 1/1/1 & -.005/.232/.965/1.074 & -.003/.189/.958/1.007 & -.009/.160/.957/1.008 & -.001/.127/.956/1.018 \\
LD-AC & RB+SL & 1/1/1 & -.006/.233/.968/1.078 & -.003/.189/.964/1.014 & -.008/.160/.959/1.011 & -.001/.127/.956/1.020 \\
\addlinespace[1.2pt]
LD-T2 & G+glmnet & 1/0/0 & -.005/.244/.965/1.148 & -.006/.193/.967/1.066 & -.007/.164/.960/1.046 & -.000/.131/.960/1.048 \\
LD-T2 & G+RF & 1/0/0 & -.005/.249/.965/1.174 & -.003/.203/.969/1.096 & -.008/.173/.968/1.096 & -.002/.139/.976/1.121 \\
LD-T2 & G+SL & 1/0/0 & -.006/.253/.982/1.396 & -.004/.203/.982/1.395 & -.005/.171/.982/1.394 & -.001/.133/.980/1.247 \\
LD-T2 & RB+glmnet & 1/0/0 & -.006/.244/.967/1.145 & -.005/.194/.966/1.061 & -.009/.164/.960/1.048 & -.001/.130/.965/1.058 \\
LD-T2 & RB+RF & 1/0/0 & -.005/.249/.970/1.174 & -.005/.203/.968/1.093 & -.008/.173/.964/1.094 & -.001/.140/.971/1.109 \\
LD-T2 & RB+SL & 1/0/0 & -.006/.253/.979/1.424 & -.006/.204/.982/1.391 & -.008/.170/.978/1.400 & .000/.133/.977/1.247 \\
\addlinespace[1.2pt]
LD-T3 & G+glmnet & 1/0/0 & -.010/.252/.969/1.113 & -.005/.200/.961/1.032 & -.010/.166/.958/1.037 & -.005/.131/.957/1.045 \\
LD-T3 & G+RF & 1/0/0 & -.011/.253/.971/1.114 & -.006/.200/.960/1.035 & -.009/.168/.959/1.034 & -.001/.130/.959/1.048 \\
LD-T3 & G+SL & 1/0/0 & -.010/.253/.975/1.165 & -.006/.202/.966/1.064 & -.011/.168/.962/1.061 & -.005/.132/.964/1.051 \\
LD-T3 & RB+glmnet & 1/0/0 & -.010/.252/.968/1.111 & -.005/.199/.963/1.033 & -.011/.167/.958/1.035 & -.005/.131/.960/1.046 \\
LD-T3 & RB+RF & 1/0/0 & -.010/.252/.970/1.117 & -.005/.201/.961/1.034 & -.010/.167/.964/1.041 & -.002/.130/.960/1.049 \\
LD-T3 & RB+SL & 1/0/0 & -.011/.253/.972/1.182 & -.007/.203/.964/1.060 & -.011/.168/.962/1.061 & -.004/.132/.963/1.050 \\
\addlinespace[1.2pt]
LD-T4 & G+glmnet & 0/0/0 & .001/.259/.971/1.144 & .005/.204/.968/1.056 & -.002/.169/.965/1.056 & .004/.132/.964/1.063 \\
LD-T4 & G+RF & 0/0/0 & .000/.260/.968/1.144 & .005/.205/.967/1.059 & -.002/.170/.961/1.056 & .006/.131/.968/1.071 \\
LD-T4 & G+SL & 0/0/0 & .000/.260/.971/1.207 & .003/.207/.968/1.097 & -.004/.171/.965/1.083 & .002/.133/.966/1.073 \\
LD-T4 & RB+glmnet & 0/0/0 & .001/.259/.969/1.140 & .005/.205/.965/1.053 & -.002/.169/.963/1.055 & .004/.132/.965/1.070 \\
LD-T4 & RB+RF & 0/0/0 & .002/.259/.973/1.150 & .005/.206/.967/1.056 & -.002/.170/.962/1.059 & .006/.131/.965/1.072 \\
LD-T4 & RB+SL & 0/0/0 & .000/.259/.973/1.218 & .003/.208/.971/1.085 & -.004/.171/.963/1.083 & .003/.133/.965/1.074 \\
\addlinespace[1.2pt]
LD-T5 & G+glmnet & 0/0/0 & -.010/.252/.968/1.118 & -.006/.200/.962/1.039 & -.010/.168/.959/1.039 & -.007/.134/.957/1.045 \\
LD-T5 & G+RF & 0/0/0 & -.009/.257/.970/1.167 & -.004/.211/.970/1.086 & -.012/.178/.968/1.112 & -.008/.142/.976/1.155 \\
LD-T5 & G+SL & 0/0/0 & -.012/.261/.980/1.400 & -.012/.211/.980/1.410 & -.020/.177/.982/1.440 & -.021/.138/.980/1.276 \\
LD-T5 & RB+glmnet & 0/0/0 & -.011/.253/.968/1.116 & -.006/.201/.961/1.033 & -.012/.169/.964/1.042 & -.007/.132/.962/1.054 \\
LD-T5 & RB+RF & 0/0/0 & -.009/.258/.971/1.154 & -.005/.212/.968/1.081 & -.013/.178/.970/1.107 & -.007/.142/.975/1.149 \\
LD-T5 & RB+SL & 0/0/0 & -.012/.260/.985/1.428 & -.012/.213/.984/1.409 & -.022/.177/.983/1.445 & -.020/.138/.976/1.280 \\
\addlinespace[1.2pt]
LD-T6 & G+glmnet & 0/0/0 & .001/.259/.970/1.147 & .004/.205/.968/1.058 & -.002/.171/.963/1.055 & .002/.134/.963/1.065 \\
LD-T6 & G+RF & 0/0/0 & .002/.264/.974/1.179 & .006/.216/.969/1.087 & -.003/.180/.972/1.118 & .001/.143/.976/1.155 \\
LD-T6 & G+SL & 0/0/0 & -.002/.268/.981/1.393 & -.003/.216/.980/1.403 & -.011/.179/.983/1.439 & -.012/.138/.983/1.284 \\
LD-T6 & RB+glmnet & 0/0/0 & .001/.261/.971/1.141 & .004/.206/.966/1.054 & -.004/.171/.964/1.054 & .001/.133/.966/1.074 \\
LD-T6 & RB+RF & 0/0/0 & .002/.265/.972/1.173 & .004/.216/.971/1.087 & -.004/.180/.971/1.110 & .002/.144/.975/1.145 \\
LD-T6 & RB+SL & 0/0/0 & -.002/.267/.983/1.425 & -.003/.216/.985/1.400 & -.013/.179/.984/1.438 & -.011/.139/.976/1.286 \\
\addlinespace[1.2pt]
LD-U2 & G+glmnet & 1/0/0 & -.008/.238/.972/1.134 & -.002/.194/.965/1.046 & -.011/.165/.959/1.037 & -.002/.131/.964/1.048 \\
LD-U2 & G+RF & 1/0/0 & -.008/.245/.976/1.151 & -.004/.203/.966/1.081 & -.010/.175/.967/1.080 & -.001/.141/.962/1.104 \\
LD-U2 & G+SL & 1/0/0 & -.007/.248/.987/1.406 & -.003/.207/.981/1.349 & -.012/.171/.984/1.389 & -.001/.134/.975/1.235 \\
LD-U2 & RB+glmnet & 1/0/0 & -.007/.238/.970/1.136 & -.003/.193/.967/1.049 & -.009/.165/.964/1.039 & -.002/.131/.963/1.043 \\
LD-U2 & RB+RF & 1/0/0 & -.006/.246/.977/1.149 & -.003/.202/.968/1.082 & -.011/.175/.968/1.080 & -.002/.139/.965/1.114 \\
LD-U2 & RB+SL & 1/0/0 & -.007/.250/.986/1.411 & -.002/.204/.978/1.377 & -.010/.172/.978/1.375 & -.003/.134/.976/1.238 \\
\addlinespace[1.2pt]
LD-U3 & G+glmnet & 1/0/0 & -.007/.240/.969/1.138 & -.004/.190/.961/1.037 & -.008/.162/.952/1.006 & .001/.128/.953/1.004 \\
LD-U3 & G+RF & 1/0/0 & -.007/.240/.966/1.140 & -.004/.191/.965/1.040 & -.009/.162/.954/1.018 & -.002/.128/.952/1.002 \\
LD-U3 & G+SL & 1/0/0 & -.009/.241/.966/1.198 & -.003/.193/.965/1.066 & -.007/.164/.955/1.034 & .001/.128/.956/1.028 \\
LD-U3 & RB+glmnet & 1/0/0 & -.006/.240/.970/1.132 & -.005/.191/.960/1.032 & -.008/.162/.953/1.011 & .001/.128/.953/1.004 \\
LD-U3 & RB+RF & 1/0/0 & -.006/.241/.966/1.136 & -.004/.191/.963/1.040 & -.009/.162/.958/1.019 & -.001/.129/.953/1.002 \\
LD-U3 & RB+SL & 1/0/0 & -.008/.241/.969/1.207 & -.003/.191/.966/1.079 & -.007/.162/.956/1.040 & .000/.128/.960/1.024 \\
\addlinespace[1.2pt]
LD-U4 & G+glmnet & 0/0/0 & -.024/.245/.968/1.139 & -.020/.193/.962/1.057 & -.025/.166/.955/1.023 & -.014/.132/.954/1.016 \\
LD-U4 & G+RF & 0/0/0 & -.024/.245/.968/1.139 & -.020/.195/.961/1.060 & -.025/.167/.958/1.030 & -.016/.132/.956/1.013 \\
LD-U4 & G+SL & 0/0/0 & -.024/.246/.971/1.204 & -.019/.197/.968/1.095 & -.022/.168/.957/1.052 & -.012/.132/.958/1.037 \\
LD-U4 & RB+glmnet & 0/0/0 & -.024/.245/.966/1.132 & -.021/.194/.964/1.050 & -.024/.166/.959/1.029 & -.014/.132/.955/1.014 \\
LD-U4 & RB+RF & 0/0/0 & -.024/.247/.964/1.131 & -.020/.194/.961/1.062 & -.025/.166/.959/1.033 & -.016/.132/.957/1.015 \\
LD-U4 & RB+SL & 0/0/0 & -.023/.247/.968/1.209 & -.018/.195/.964/1.102 & -.022/.168/.958/1.051 & -.013/.132/.958/1.036 \\
\addlinespace[1.2pt]
LD-U5 & G+glmnet & 0/0/0 & -.007/.241/.969/1.137 & -.003/.192/.961/1.036 & -.008/.164/.952/1.011 & .004/.131/.954/1.009 \\
LD-U5 & G+RF & 0/0/0 & -.010/.250/.965/1.160 & -.007/.201/.970/1.104 & -.009/.177/.961/1.078 & .002/.143/.959/1.088 \\
LD-U5 & G+SL & 0/0/0 & -.008/.251/.980/1.457 & .001/.205/.982/1.421 & -.001/.170/.987/1.442 & .015/.135/.976/1.254 \\
LD-U5 & RB+glmnet & 0/0/0 & -.006/.240/.969/1.139 & -.003/.190/.959/1.042 & -.006/.164/.955/1.016 & .004/.131/.950/1.003 \\
LD-U5 & RB+RF & 0/0/0 & -.009/.249/.967/1.162 & -.006/.200/.970/1.106 & -.008/.177/.964/1.073 & .001/.141/.964/1.106 \\
LD-U5 & RB+SL & 0/0/0 & -.007/.254/.982/1.452 & .001/.200/.985/1.455 & .001/.171/.978/1.438 & .014/.135/.977/1.250 \\
\addlinespace[1.2pt]
LD-U6 & G+glmnet & 0/0/0 & -.024/.246/.967/1.137 & -.019/.195/.962/1.052 & -.025/.167/.954/1.029 & -.012/.134/.952/1.018 \\
LD-U6 & G+RF & 0/0/0 & -.025/.255/.968/1.152 & -.022/.204/.964/1.095 & -.024/.179/.957/1.082 & -.012/.145/.957/1.089 \\
LD-U6 & G+SL & 0/0/0 & -.022/.254/.982/1.415 & -.013/.207/.984/1.401 & -.016/.173/.982/1.431 & .000/.136/.971/1.246 \\
LD-U6 & RB+glmnet & 0/0/0 & -.024/.246/.967/1.136 & -.020/.194/.961/1.058 & -.023/.167/.958/1.031 & -.012/.134/.952/1.014 \\
LD-U6 & RB+RF & 0/0/0 & -.025/.254/.966/1.151 & -.020/.204/.964/1.098 & -.023/.178/.962/1.081 & -.013/.142/.963/1.105 \\
LD-U6 & RB+SL & 0/0/0 & -.022/.258/.982/1.411 & -.014/.204/.982/1.428 & -.014/.174/.980/1.416 & -.001/.136/.975/1.242 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Low-dimensional-study performance for the ISME, $W_i=1$.}\label{tab:sim-ld-ISME-C}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
LD-AC & G+glmnet & 1/1/1 & .000/.151/.960/1.324 & -.001/.110/.958/1.184 & -.001/.093/.949/1.081 & -.000/.070/.951/1.069 \\
LD-AC & G+RF & 1/1/1 & .000/.151/.959/1.335 & -.001/.110/.964/1.207 & -.001/.094/.953/1.101 & .001/.070/.951/1.073 \\
LD-AC & G+SL & 1/1/1 & .001/.151/.962/1.437 & -.002/.111/.966/1.258 & -.001/.094/.953/1.161 & .001/.071/.949/1.108 \\
LD-AC & RB+glmnet & 1/1/1 & .000/.151/.957/1.317 & -.001/.110/.959/1.184 & -.001/.093/.950/1.092 & .001/.070/.948/1.070 \\
LD-AC & RB+RF & 1/1/1 & -.001/.152/.960/1.328 & -.001/.111/.963/1.196 & -.001/.094/.952/1.100 & .000/.070/.956/1.080 \\
LD-AC & RB+SL & 1/1/1 & .000/.152/.961/1.429 & -.001/.113/.955/1.234 & -.001/.094/.951/1.151 & .000/.070/.950/1.118 \\
\addlinespace[1.2pt]
LD-T2 & G+glmnet & 1/0/0 & -.001/.152/.958/1.319 & -.000/.112/.958/1.181 & -.003/.096/.946/1.080 & .000/.073/.950/1.058 \\
LD-T2 & G+RF & 1/0/0 & -.001/.165/.968/1.316 & -.002/.128/.966/1.202 & -.001/.113/.960/1.135 & .001/.091/.969/1.172 \\
LD-T2 & G+SL & 1/0/0 & .000/.167/.980/1.697 & -.002/.131/.984/1.676 & -.004/.106/.980/1.673 & .001/.078/.978/1.421 \\
LD-T2 & RB+glmnet & 1/0/0 & .000/.152/.960/1.323 & -.001/.112/.962/1.180 & -.001/.096/.946/1.079 & .000/.073/.951/1.059 \\
LD-T2 & RB+RF & 1/0/0 & -.001/.167/.957/1.296 & -.001/.129/.968/1.191 & -.002/.113/.967/1.136 & .001/.090/.974/1.182 \\
LD-T2 & RB+SL & 1/0/0 & -.000/.171/.978/1.706 & -.000/.130/.983/1.709 & -.002/.107/.979/1.658 & .000/.079/.979/1.415 \\
\addlinespace[1.2pt]
LD-T3 & G+glmnet & 1/0/0 & -.010/.158/.961/1.317 & -.010/.114/.960/1.190 & -.010/.098/.942/1.077 & -.006/.073/.950/1.076 \\
LD-T3 & G+RF & 1/0/0 & -.009/.159/.956/1.322 & -.010/.115/.960/1.199 & -.010/.099/.947/1.096 & -.009/.074/.950/1.076 \\
LD-T3 & G+SL & 1/0/0 & -.008/.161/.962/1.461 & -.008/.119/.963/1.279 & -.007/.100/.952/1.157 & -.004/.074/.952/1.126 \\
LD-T3 & RB+glmnet & 1/0/0 & -.010/.158/.959/1.303 & -.011/.115/.958/1.182 & -.009/.097/.944/1.086 & -.005/.073/.949/1.082 \\
LD-T3 & RB+RF & 1/0/0 & -.010/.160/.960/1.308 & -.010/.116/.962/1.193 & -.009/.099/.944/1.090 & -.009/.073/.951/1.080 \\
LD-T3 & RB+SL & 1/0/0 & -.007/.162/.961/1.486 & -.007/.120/.962/1.261 & -.007/.100/.953/1.149 & -.005/.074/.952/1.127 \\
\addlinespace[1.2pt]
LD-T4 & G+glmnet & 1/0/0 & -.010/.158/.961/1.317 & -.010/.114/.960/1.190 & -.010/.098/.942/1.077 & -.006/.073/.950/1.076 \\
LD-T4 & G+RF & 1/0/0 & -.009/.159/.956/1.322 & -.010/.115/.960/1.199 & -.010/.099/.947/1.096 & -.009/.074/.950/1.076 \\
LD-T4 & G+SL & 1/0/0 & -.008/.161/.962/1.461 & -.008/.119/.963/1.279 & -.007/.100/.952/1.157 & -.004/.074/.952/1.126 \\
LD-T4 & RB+glmnet & 1/0/0 & -.010/.158/.959/1.303 & -.011/.115/.958/1.182 & -.009/.097/.944/1.086 & -.005/.073/.949/1.082 \\
LD-T4 & RB+RF & 1/0/0 & -.010/.160/.960/1.308 & -.010/.116/.962/1.193 & -.009/.099/.944/1.090 & -.009/.073/.951/1.080 \\
LD-T4 & RB+SL & 1/0/0 & -.007/.162/.961/1.486 & -.007/.120/.962/1.261 & -.007/.100/.953/1.149 & -.005/.074/.952/1.127 \\
\addlinespace[1.2pt]
LD-T5 & G+glmnet & 0/0/0 & -.010/.159/.961/1.307 & -.009/.116/.958/1.179 & -.010/.100/.940/1.074 & -.004/.077/.948/1.051 \\
LD-T5 & G+RF & 0/0/0 & -.009/.174/.962/1.295 & -.010/.136/.967/1.189 & -.006/.120/.960/1.129 & -.003/.095/.969/1.183 \\
LD-T5 & G+SL & 0/0/0 & -.005/.175/.976/1.672 & -.001/.137/.983/1.682 & .002/.112/.982/1.704 & .011/.084/.979/1.433 \\
LD-T5 & RB+glmnet & 0/0/0 & -.010/.159/.958/1.306 & -.009/.116/.962/1.184 & -.008/.100/.943/1.073 & -.004/.077/.948/1.050 \\
LD-T5 & RB+RF & 0/0/0 & -.010/.176/.961/1.279 & -.009/.135/.969/1.191 & -.007/.120/.960/1.130 & -.004/.094/.973/1.197 \\
LD-T5 & RB+SL & 0/0/0 & -.006/.179/.979/1.682 & -.001/.135/.985/1.722 & .004/.113/.978/1.681 & .010/.084/.979/1.428 \\
\addlinespace[1.2pt]
LD-T6 & G+glmnet & 0/0/0 & -.010/.159/.961/1.307 & -.009/.116/.958/1.179 & -.010/.100/.940/1.074 & -.004/.077/.948/1.051 \\
LD-T6 & G+RF & 0/0/0 & -.009/.174/.962/1.295 & -.010/.136/.967/1.189 & -.006/.120/.960/1.129 & -.003/.095/.969/1.183 \\
LD-T6 & G+SL & 0/0/0 & -.005/.175/.976/1.672 & -.001/.137/.983/1.682 & .002/.112/.982/1.704 & .011/.084/.979/1.433 \\
LD-T6 & RB+glmnet & 0/0/0 & -.010/.159/.958/1.306 & -.009/.116/.962/1.184 & -.008/.100/.943/1.073 & -.004/.077/.948/1.050 \\
LD-T6 & RB+RF & 0/0/0 & -.010/.176/.961/1.279 & -.009/.135/.969/1.191 & -.007/.120/.960/1.130 & -.004/.094/.973/1.197 \\
LD-T6 & RB+SL & 0/0/0 & -.006/.179/.979/1.682 & -.001/.135/.985/1.722 & .004/.113/.978/1.681 & .010/.084/.979/1.428 \\
\addlinespace[1.2pt]
LD-U2 & G+glmnet & 1/0/0 & .002/.141/.953/1.182 & -.003/.104/.946/1.058 & .001/.090/.933/.985 & .001/.068/.941/1.002 \\
LD-U2 & G+RF & 1/0/0 & .002/.151/.953/1.211 & -.000/.118/.962/1.154 & .001/.103/.964/1.149 & .001/.084/.973/1.207 \\
LD-U2 & G+SL & 1/0/0 & .002/.162/.975/1.704 & -.002/.121/.976/1.815 & .003/.099/.978/1.842 & .002/.074/.977/1.526 \\
LD-U2 & RB+glmnet & 1/0/0 & .001/.143/.954/1.176 & -.002/.104/.946/1.060 & -.000/.089/.936/.989 & .002/.069/.940/1.002 \\
LD-U2 & RB+RF & 1/0/0 & .000/.152/.954/1.212 & -.002/.118/.957/1.144 & .001/.104/.963/1.130 & .002/.085/.970/1.195 \\
LD-U2 & RB+SL & 1/0/0 & .001/.160/.973/1.748 & -.003/.124/.983/1.789 & .000/.099/.980/1.848 & .002/.073/.983/1.550 \\
\addlinespace[1.2pt]
LD-U3 & G+glmnet & 1/0/0 & .001/.159/.972/1.377 & -.000/.120/.967/1.213 & -.002/.101/.966/1.135 & -.002/.077/.964/1.115 \\
LD-U3 & G+RF & 1/0/0 & .001/.160/.973/1.382 & -.001/.122/.969/1.223 & -.001/.103/.968/1.150 & .002/.077/.963/1.126 \\
LD-U3 & G+SL & 1/0/0 & .003/.163/.973/1.525 & -.002/.125/.968/1.288 & -.002/.103/.968/1.229 & -.000/.078/.960/1.157 \\
LD-U3 & RB+glmnet & 1/0/0 & .001/.159/.973/1.365 & -.000/.120/.967/1.211 & -.001/.101/.965/1.143 & -.001/.077/.964/1.116 \\
LD-U3 & RB+RF & 1/0/0 & .000/.160/.973/1.377 & -.000/.122/.971/1.218 & -.001/.102/.969/1.161 & .001/.076/.968/1.136 \\
LD-U3 & RB+SL & 1/0/0 & .002/.163/.977/1.536 & -.001/.127/.970/1.275 & -.003/.103/.965/1.227 & -.001/.078/.963/1.173 \\
\addlinespace[1.2pt]
LD-U4 & G+glmnet & 0/0/0 & .018/.150/.966/1.208 & .016/.113/.960/1.091 & .015/.096/.955/1.033 & .014/.073/.961/1.056 \\
LD-U4 & G+RF & 0/0/0 & .018/.151/.967/1.210 & .016/.114/.962/1.104 & .015/.097/.953/1.043 & .016/.072/.960/1.071 \\
LD-U4 & G+SL & 0/0/0 & .019/.154/.966/1.364 & .014/.116/.967/1.197 & .013/.098/.958/1.105 & .012/.073/.956/1.094 \\
LD-U4 & RB+glmnet & 0/0/0 & .018/.150/.966/1.200 & .016/.113/.961/1.086 & .015/.096/.952/1.033 & .014/.072/.959/1.063 \\
LD-U4 & RB+RF & 0/0/0 & .018/.151/.964/1.213 & .016/.115/.966/1.096 & .015/.097/.953/1.051 & .016/.072/.962/1.072 \\
LD-U4 & RB+SL & 0/0/0 & .018/.153/.971/1.395 & .013/.119/.962/1.177 & .012/.097/.955/1.105 & .013/.073/.961/1.096 \\
\addlinespace[1.2pt]
LD-U5 & G+glmnet & 0/0/0 & .001/.159/.975/1.380 & -.002/.121/.968/1.211 & -.002/.102/.968/1.140 & -.004/.079/.964/1.115 \\
LD-U5 & G+RF & 0/0/0 & .004/.167/.968/1.394 & .003/.136/.972/1.285 & -.000/.116/.975/1.288 & -.002/.094/.983/1.313 \\
LD-U5 & G+SL & 0/0/0 & .003/.175/.978/1.863 & -.006/.137/.986/1.915 & -.009/.112/.987/1.959 & -.015/.086/.990/1.631 \\
LD-U5 & RB+glmnet & 0/0/0 & .001/.160/.973/1.371 & -.001/.121/.969/1.208 & -.003/.102/.969/1.147 & -.004/.078/.966/1.125 \\
LD-U5 & RB+RF & 0/0/0 & .003/.166/.971/1.400 & .002/.136/.966/1.275 & -.001/.118/.975/1.261 & -.001/.094/.985/1.325 \\
LD-U5 & RB+SL & 0/0/0 & .001/.172/.981/1.905 & -.005/.139/.988/1.886 & -.011/.113/.988/1.962 & -.014/.084/.988/1.656 \\
\addlinespace[1.2pt]
LD-U6 & G+glmnet & 0/0/0 & .019/.150/.964/1.214 & .015/.114/.963/1.087 & .015/.098/.955/1.039 & .012/.074/.966/1.068 \\
LD-U6 & G+RF & 0/0/0 & .019/.160/.966/1.245 & .017/.130/.965/1.164 & .014/.111/.972/1.208 & .012/.090/.976/1.262 \\
LD-U6 & G+SL & 0/0/0 & .017/.170/.980/1.709 & .008/.132/.982/1.819 & .007/.107/.983/1.885 & -.000/.079/.986/1.601 \\
LD-U6 & RB+glmnet & 0/0/0 & .018/.151/.966/1.198 & .015/.114/.959/1.089 & .014/.098/.950/1.038 & .012/.073/.962/1.081 \\
LD-U6 & RB+RF & 0/0/0 & .019/.159/.963/1.252 & .016/.130/.964/1.161 & .014/.113/.967/1.171 & .013/.091/.981/1.257 \\
LD-U6 & RB+SL & 0/0/0 & .016/.166/.981/1.767 & .009/.133/.986/1.805 & .005/.109/.981/1.868 & .001/.078/.986/1.616 \\
\bottomrule
\end{longtable}
}
\end{landscape}



==> final_results/report/simulation_tables_individual.tex <==
% Generated from final_results(0828)/annals_simulation_bundle.rds.
% Each numerical cell is bias/RMSE/coverage/mean-SE-to-empirical-SD.
% P/AL/CI separately records point consistency, asymptotic linearity,
% and confidence-interval validity under the stated theoretical limit.

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Canonical-study performance for the IDE, $W_i=N_i$.}\label{tab:sim-can-IDE-I}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
C-1111 & Can-par & 1/1/1 & .003/.269/.948/.991 & .007/.212/.943/.992 & .006/.179/.954/1.008 & .003/.144/.951/1.008 \\
C-1111 & Can-SL & 1/1/1 & .001/.283/.953/1.152 & .006/.223/.950/1.044 & .006/.185/.954/1.057 & .002/.147/.955/1.038 \\
C-1111 & g-comp & 1/1/1 & .002/.237/.953/1.214 & .004/.193/.943/1.012 & .005/.163/.944/1.015 & .003/.130/.942/1.017 \\
\addlinespace[1.2pt]
C-1110 & Can-par & 1/0/0 & .001/.292/.984/1.341 & .004/.235/.983/1.393 & .005/.201/.990/1.449 & .003/.164/.992/1.511 \\
C-1110 & Can-SL & 1/0/0 & -.001/.299/.977/1.315 & .005/.241/.982/1.361 & .005/.204/.988/1.425 & .003/.165/.993/1.492 \\
C-1110 & g-comp & 1/1/1 & .002/.237/.953/1.214 & .004/.193/.943/1.012 & .005/.163/.944/1.015 & .003/.130/.942/1.017 \\
\addlinespace[1.2pt]
C-1101 & Can-par & 1/0/0 & .000/.301/.927/.962 & .010/.239/.926/.929 & .009/.207/.923/.920 & .006/.166/.924/.919 \\
C-1101 & Can-SL & 1/0/0 & .008/.311/.944/1.225 & .016/.247/.939/1.051 & .015/.212/.941/1.023 & .009/.172/.937/.976 \\
C-1101 & g-comp & 0/0/0 & .084/.264/.942/1.208 & .087/.219/.926/1.019 & .086/.189/.911/1.025 & .087/.161/.902/1.019 \\
\addlinespace[1.2pt]
C-1100 & Can-par & 1/0/0 & -.000/.286/.952/1.038 & .007/.229/.953/1.046 & .005/.197/.959/1.076 & .008/.161/.961/1.087 \\
C-1100 & Can-SL & 1/0/0 & .007/.288/.948/1.027 & .012/.230/.951/1.034 & .010/.198/.956/1.061 & .011/.161/.958/1.071 \\
C-1100 & g-comp & 0/0/0 & .084/.264/.942/1.208 & .087/.219/.926/1.019 & .086/.189/.911/1.025 & .087/.161/.902/1.019 \\
\addlinespace[1.2pt]
C-1011 & Can-par & 1/0/0 & -.019/.558/.949/.958 & .009/.442/.953/.977 & .002/.381/.953/.970 & -.005/.300/.957/1.003 \\
C-1011 & Can-SL & 1/0/0 & -.019/.551/.959/1.034 & .011/.442/.957/1.000 & .003/.380/.954/.989 & -.004/.299/.958/1.014 \\
C-1011 & g-comp & 0/0/0 & .069/.450/.958/1.156 & .092/.372/.928/1.001 & .082/.320/.928/.989 & .089/.257/.936/1.024 \\
\addlinespace[1.2pt]
C-1010 & Can-par & 1/0/0 & -.021/.568/.969/1.077 & .006/.452/.975/1.111 & .001/.392/.972/1.116 & -.004/.312/.978/1.169 \\
C-1010 & Can-SL & 1/0/0 & -.021/.555/.968/1.104 & .009/.449/.979/1.124 & .002/.390/.976/1.120 & -.003/.310/.978/1.172 \\
C-1010 & g-comp & 0/0/0 & .069/.450/.958/1.156 & .092/.372/.928/1.001 & .082/.320/.928/.989 & .089/.257/.936/1.024 \\
\addlinespace[1.2pt]
C-1001 & Can-par & 0/0/0 & .087/.471/.938/.961 & .110/.383/.936/.945 & .099/.331/.929/.944 & .094/.265/.935/.963 \\
C-1001 & Can-SL & 0/0/0 & .091/.475/.953/1.112 & .114/.391/.936/1.003 & .102/.335/.941/.993 & .096/.270/.941/.990 \\
C-1001 & g-comp & 0/0/0 & .054/.421/.962/1.186 & .082/.347/.930/1.012 & .074/.299/.929/.995 & .084/.241/.932/1.022 \\
\addlinespace[1.2pt]
C-1000 & Can-par & 0/0/0 & .086/.460/.945/.990 & .107/.375/.949/.998 & .095/.325/.954/1.005 & .096/.264/.949/1.030 \\
C-1000 & Can-SL & 0/0/0 & .090/.457/.949/.997 & .109/.375/.948/.996 & .098/.327/.950/.996 & .097/.265/.947/1.024 \\
C-1000 & g-comp & 0/0/0 & .054/.421/.962/1.186 & .082/.347/.930/1.012 & .074/.299/.929/.995 & .084/.241/.932/1.022 \\
\addlinespace[1.2pt]
C-0111 & Can-par & 1/0/0 & .007/.276/.944/.985 & .007/.218/.944/.992 & .007/.185/.951/1.002 & .002/.149/.949/1.002 \\
C-0111 & Can-SL & 1/0/0 & .002/.292/.949/1.159 & .006/.230/.949/1.059 & .007/.194/.957/1.048 & .002/.154/.954/1.035 \\
C-0111 & g-comp & 0/0/0 & .003/.238/.948/1.051 & .002/.191/.938/1.014 & .003/.164/.942/1.005 & .001/.131/.943/1.017 \\
\addlinespace[1.2pt]
C-0110 & Can-par & 0/0/0 & .000/.300/.984/1.335 & .000/.241/.988/1.430 & .001/.211/.993/1.474 & -.003/.173/.994/1.551 \\
C-0110 & Can-SL & 0/0/0 & -.007/.314/.979/1.306 & -.001/.253/.986/1.395 & -.002/.218/.993/1.448 & -.005/.176/.992/1.532 \\
C-0110 & g-comp & 0/0/0 & .003/.238/.948/1.051 & .002/.191/.938/1.014 & .003/.164/.942/1.005 & .001/.131/.943/1.017 \\
\addlinespace[1.2pt]
C-0101 & Can-par & 0/0/0 & .007/.296/.929/.977 & .010/.238/.936/.943 & .011/.208/.934/.929 & .007/.169/.928/.932 \\
C-0101 & Can-SL & 0/0/0 & .007/.304/.951/1.267 & .012/.248/.951/1.065 & .013/.215/.944/1.030 & .010/.175/.940/.992 \\
C-0101 & g-comp & 0/0/0 & .081/.258/.929/1.045 & .084/.213/.921/1.017 & .084/.186/.910/1.018 & .084/.158/.900/1.018 \\
\addlinespace[1.2pt]
C-0100 & Can-par & 0/0/0 & .005/.284/.953/1.036 & .007/.229/.956/1.056 & .005/.200/.959/1.075 & .005/.162/.965/1.096 \\
C-0100 & Can-SL & 0/0/0 & .005/.289/.949/1.028 & .008/.230/.952/1.047 & .007/.202/.958/1.057 & .007/.163/.962/1.078 \\
C-0100 & g-comp & 0/0/0 & .081/.258/.929/1.045 & .084/.213/.921/1.017 & .084/.186/.910/1.018 & .084/.158/.900/1.018 \\
\addlinespace[1.2pt]
C-0011 & Can-par & 1/0/0 & -.016/.595/.949/.969 & .009/.480/.957/.977 & .002/.418/.950/.969 & -.005/.329/.955/1.003 \\
C-0011 & Can-SL & 1/0/0 & -.019/.601/.959/1.039 & .011/.486/.958/1.006 & .003/.420/.952/.991 & -.004/.332/.956/1.015 \\
C-0011 & g-comp & 0/0/0 & .069/.485/.935/1.003 & .092/.405/.926/.978 & .080/.350/.922/.976 & .085/.280/.928/1.009 \\
\addlinespace[1.2pt]
C-0010 & Can-par & 0/0/0 & -.022/.606/.972/1.099 & .003/.492/.980/1.137 & -.005/.430/.975/1.147 & -.010/.343/.977/1.209 \\
C-0010 & Can-SL & 0/0/0 & -.027/.612/.977/1.105 & .005/.498/.977/1.144 & -.007/.433/.980/1.153 & -.011/.345/.979/1.212 \\
C-0010 & g-comp & 0/0/0 & .069/.485/.935/1.003 & .092/.405/.926/.978 & .080/.350/.922/.976 & .085/.280/.928/1.009 \\
\addlinespace[1.2pt]
C-0001 & Can-par & 0/0/0 & .095/.502/.953/.978 & .113/.418/.930/.948 & .100/.363/.930/.946 & .096/.296/.928/.955 \\
C-0001 & Can-SL & 0/0/0 & .097/.516/.957/1.120 & .115/.431/.938/1.000 & .101/.371/.939/.989 & .098/.301/.932/.982 \\
C-0001 & g-comp & 0/0/0 & .049/.452/.942/1.014 & .078/.374/.929/.989 & .071/.326/.925/.981 & .079/.261/.927/1.010 \\
\addlinespace[1.2pt]
C-0000 & Can-par & 0/0/0 & .094/.495/.948/.995 & .109/.410/.941/.991 & .094/.358/.949/.997 & .094/.291/.944/1.019 \\
C-0000 & Can-SL & 0/0/0 & .095/.505/.948/.997 & .111/.417/.941/.987 & .095/.364/.947/.986 & .095/.293/.942/1.015 \\
C-0000 & g-comp & 0/0/0 & .049/.452/.942/1.014 & .078/.374/.929/.989 & .071/.326/.925/.981 & .079/.261/.927/1.010 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Canonical-study performance for the IIME, $W_i=N_i$.}\label{tab:sim-can-IIME-I}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
C-1111 & Can-par & 1/1/1 & -.005/.238/.963/.999 & -.004/.194/.955/.979 & -.010/.165/.950/.991 & -.001/.131/.956/1.013 \\
C-1111 & Can-SL & 1/1/1 & -.010/.235/.958/.990 & -.006/.193/.950/.970 & -.009/.165/.954/.986 & -.002/.131/.955/1.010 \\
C-1111 & g-comp & 1/1/1 & -.001/.188/.946/1.043 & .002/.155/.936/.994 & .001/.134/.939/.981 & .002/.105/.940/1.014 \\
\addlinespace[1.2pt]
C-1110 & Can-par & 1/0/0 & -.006/.237/.964/1.007 & -.004/.193/.956/.987 & -.009/.165/.952/.999 & -.002/.131/.961/1.024 \\
C-1110 & Can-SL & 1/0/0 & -.011/.233/.958/.994 & -.006/.192/.957/.979 & -.010/.164/.954/.993 & -.002/.131/.959/1.019 \\
C-1110 & g-comp & 1/1/1 & -.001/.188/.946/1.043 & .002/.155/.936/.994 & .001/.134/.939/.981 & .002/.105/.940/1.014 \\
\addlinespace[1.2pt]
C-1101 & Can-par & 0/0/0 & -.078/.400/.949/.971 & -.061/.324/.946/.980 & -.075/.288/.942/.965 & -.069/.235/.944/.986 \\
C-1101 & Can-SL & 0/0/0 & -.088/.390/.946/.962 & -.066/.319/.943/.973 & -.078/.285/.940/.962 & -.071/.233/.944/.986 \\
C-1101 & g-comp & 0/0/0 & -.070/.276/.933/1.043 & -.058/.237/.923/.979 & -.066/.208/.916/.976 & -.063/.168/.925/1.009 \\
\addlinespace[1.2pt]
C-1100 & Can-par & 0/0/0 & -.077/.401/.948/.974 & -.061/.325/.949/.981 & -.074/.289/.946/.966 & -.070/.235/.945/.991 \\
C-1100 & Can-SL & 0/0/0 & -.088/.391/.943/.959 & -.066/.320/.945/.973 & -.078/.285/.940/.963 & -.071/.233/.942/.989 \\
C-1100 & g-comp & 0/0/0 & -.070/.276/.933/1.043 & -.058/.237/.923/.979 & -.066/.208/.916/.976 & -.063/.168/.925/1.009 \\
\addlinespace[1.2pt]
C-1011 & Can-par & 1/0/0 & -.008/.202/.958/.999 & -.002/.167/.956/.967 & -.006/.141/.956/.981 & -.000/.111/.958/1.009 \\
C-1011 & Can-SL & 1/0/0 & -.014/.204/.952/.983 & -.006/.170/.946/.948 & -.007/.144/.945/.963 & -.001/.113/.954/.995 \\
C-1011 & g-comp & 0/0/0 & -.003/.188/.948/1.051 & .001/.156/.938/.998 & -.000/.136/.936/.980 & .002/.106/.940/1.012 \\
\addlinespace[1.2pt]
C-1010 & Can-par & 1/0/0 & -.008/.201/.961/1.010 & -.002/.167/.957/.977 & -.005/.141/.954/.990 & -.001/.111/.957/1.025 \\
C-1010 & Can-SL & 1/0/0 & -.015/.203/.956/.988 & -.006/.169/.951/.958 & -.007/.143/.949/.971 & -.002/.112/.955/1.009 \\
C-1010 & g-comp & 0/0/0 & -.003/.188/.948/1.051 & .001/.156/.938/.998 & -.000/.136/.936/.980 & .002/.106/.940/1.012 \\
\addlinespace[1.2pt]
C-1001 & Can-par & 0/0/0 & -.093/.328/.928/.993 & -.071/.272/.929/.965 & -.080/.238/.922/.967 & -.072/.194/.915/.989 \\
C-1001 & Can-SL & 0/0/0 & -.104/.329/.920/.977 & -.079/.275/.925/.951 & -.085/.240/.911/.961 & -.074/.195/.914/.982 \\
C-1001 & g-comp & 0/0/0 & -.057/.291/.933/1.035 & -.049/.250/.921/.979 & -.060/.218/.919/.977 & -.058/.176/.928/1.007 \\
\addlinespace[1.2pt]
C-1000 & Can-par & 0/0/0 & -.092/.328/.928/.999 & -.070/.273/.929/.967 & -.079/.239/.926/.970 & -.072/.194/.914/.996 \\
C-1000 & Can-SL & 0/0/0 & -.104/.330/.922/.974 & -.078/.276/.925/.949 & -.085/.241/.916/.963 & -.074/.195/.913/.986 \\
C-1000 & g-comp & 0/0/0 & -.057/.291/.933/1.035 & -.049/.250/.921/.979 & -.060/.218/.919/.977 & -.058/.176/.928/1.007 \\
\addlinespace[1.2pt]
C-0111 & Can-par & 1/0/0 & -.010/.231/.958/.995 & -.006/.189/.954/.970 & -.011/.161/.951/.983 & -.003/.128/.952/.998 \\
C-0111 & Can-SL & 1/0/0 & -.018/.230/.955/.993 & -.011/.190/.948/.961 & -.013/.161/.950/.978 & -.004/.128/.952/.996 \\
C-0111 & g-comp & 0/0/0 & -.020/.182/.946/1.041 & -.018/.150/.935/.994 & -.019/.130/.929/.981 & -.017/.101/.943/1.016 \\
\addlinespace[1.2pt]
C-0110 & Can-par & 0/0/0 & -.015/.230/.961/1.003 & -.012/.188/.957/.982 & -.017/.160/.951/.995 & -.010/.127/.959/1.018 \\
C-0110 & Can-SL & 0/0/0 & -.021/.229/.957/.995 & -.016/.189/.954/.973 & -.019/.161/.951/.988 & -.012/.127/.956/1.013 \\
C-0110 & g-comp & 0/0/0 & -.020/.182/.946/1.041 & -.018/.150/.935/.994 & -.019/.130/.929/.981 & -.017/.101/.943/1.016 \\
\addlinespace[1.2pt]
C-0101 & Can-par & 0/0/0 & -.118/.389/.940/.981 & -.099/.318/.943/.984 & -.110/.286/.932/.971 & -.104/.237/.930/.989 \\
C-0101 & Can-SL & 0/0/0 & -.125/.383/.940/.978 & -.103/.314/.940/.982 & -.113/.283/.927/.969 & -.104/.235/.922/.990 \\
C-0101 & g-comp & 0/0/0 & -.121/.287/.919/1.037 & -.110/.249/.905/.978 & -.118/.225/.875/.977 & -.116/.191/.862/1.007 \\
\addlinespace[1.2pt]
C-0100 & Can-par & 0/0/0 & -.119/.389/.945/.983 & -.101/.318/.945/.988 & -.112/.287/.929/.973 & -.107/.238/.927/.997 \\
C-0100 & Can-SL & 0/0/0 & -.126/.384/.940/.976 & -.105/.315/.943/.983 & -.115/.284/.927/.970 & -.108/.236/.921/.995 \\
C-0100 & g-comp & 0/0/0 & -.121/.287/.919/1.037 & -.110/.249/.905/.978 & -.118/.225/.875/.977 & -.116/.191/.862/1.007 \\
\addlinespace[1.2pt]
C-0011 & Can-par & 1/0/0 & -.013/.197/.954/.991 & -.004/.163/.953/.953 & -.006/.138/.947/.962 & -.002/.109/.952/.982 \\
C-0011 & Can-SL & 1/0/0 & -.022/.201/.949/.986 & -.011/.167/.946/.937 & -.010/.141/.942/.948 & -.004/.111/.947/.972 \\
C-0011 & g-comp & 0/0/0 & -.022/.183/.945/1.049 & -.018/.152/.936/1.000 & -.020/.132/.927/.981 & -.018/.103/.938/1.013 \\
\addlinespace[1.2pt]
C-0010 & Can-par & 0/0/0 & -.019/.196/.955/1.002 & -.010/.162/.956/.969 & -.013/.138/.948/.980 & -.009/.108/.956/1.012 \\
C-0010 & Can-SL & 0/0/0 & -.026/.200/.952/.990 & -.016/.166/.950/.952 & -.016/.141/.943/.963 & -.011/.110/.951/.997 \\
C-0010 & g-comp & 0/0/0 & -.022/.183/.945/1.049 & -.018/.152/.936/1.000 & -.020/.132/.927/.981 & -.018/.103/.938/1.013 \\
\addlinespace[1.2pt]
C-0001 & Can-par & 0/0/0 & -.135/.331/.913/.996 & -.110/.277/.913/.963 & -.116/.245/.883/.969 & -.106/.203/.880/.988 \\
C-0001 & Can-SL & 0/0/0 & -.144/.337/.911/.989 & -.117/.282/.910/.955 & -.120/.248/.880/.965 & -.108/.205/.878/.982 \\
C-0001 & g-comp & 0/0/0 & -.106/.301/.920/1.028 & -.100/.261/.908/.978 & -.111/.234/.888/.978 & -.111/.198/.878/1.005 \\
\addlinespace[1.2pt]
C-0000 & Can-par & 0/0/0 & -.136/.332/.918/1.004 & -.112/.278/.913/.970 & -.117/.245/.891/.979 & -.110/.204/.876/1.002 \\
C-0000 & Can-SL & 0/0/0 & -.145/.338/.912/.991 & -.119/.283/.905/.956 & -.123/.249/.880/.972 & -.112/.206/.876/.991 \\
C-0000 & g-comp & 0/0/0 & -.106/.301/.920/1.028 & -.100/.261/.908/.978 & -.111/.234/.888/.978 & -.111/.198/.878/1.005 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Canonical-study performance for the ISME, $W_i=N_i$.}\label{tab:sim-can-ISME-I}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
C-1111 & Can-par & 1/1/1 & .001/.138/.915/.981 & -.001/.102/.919/.989 & .000/.087/.928/.986 & .002/.066/.940/1.005 \\
C-1111 & Can-SL & 1/1/1 & -.001/.145/.928/1.112 & .000/.107/.924/1.062 & .000/.091/.924/1.036 & .003/.068/.946/1.052 \\
C-1111 & g-comp & 1/1/1 & -.002/.111/.946/1.265 & -.003/.087/.938/1.060 & -.001/.076/.932/.999 & .000/.058/.942/1.035 \\
\addlinespace[1.2pt]
C-1110 & Can-par & 1/0/0 & .003/.136/.950/1.168 & -.003/.102/.957/1.239 & .001/.088/.960/1.217 & .002/.068/.973/1.299 \\
C-1110 & Can-SL & 1/0/0 & .001/.141/.946/1.191 & -.001/.104/.957/1.247 & .001/.091/.964/1.227 & .003/.069/.975/1.322 \\
C-1110 & g-comp & 1/1/1 & -.002/.111/.946/1.265 & -.003/.087/.938/1.060 & -.001/.076/.932/.999 & .000/.058/.942/1.035 \\
\addlinespace[1.2pt]
C-1101 & Can-par & 0/0/0 & .066/.184/.927/.897 & .065/.146/.930/.912 & .062/.131/.916/.880 & .064/.110/.900/.920 \\
C-1101 & Can-SL & 0/0/0 & .065/.182/.944/.959 & .065/.145/.936/.947 & .060/.130/.919/.901 & .063/.109/.907/.939 \\
C-1101 & g-comp & 0/0/0 & .060/.169/.964/1.190 & .063/.139/.937/1.050 & .058/.122/.925/1.007 & .063/.106/.896/1.016 \\
\addlinespace[1.2pt]
C-1100 & Can-par & 0/0/0 & .065/.185/.941/.921 & .064/.145/.947/.966 & .061/.130/.935/.930 & .064/.110/.917/.976 \\
C-1100 & Can-SL & 0/0/0 & .067/.184/.948/.942 & .065/.144/.945/.974 & .060/.130/.934/.926 & .064/.110/.918/.977 \\
C-1100 & g-comp & 0/0/0 & .060/.169/.964/1.190 & .063/.139/.937/1.050 & .058/.122/.925/1.007 & .063/.106/.896/1.016 \\
\addlinespace[1.2pt]
C-1011 & Can-par & 1/0/0 & .001/.138/.915/.981 & -.001/.102/.919/.989 & .000/.087/.928/.986 & .002/.066/.940/1.005 \\
C-1011 & Can-SL & 1/0/0 & -.001/.145/.928/1.112 & .001/.107/.924/1.062 & .000/.091/.925/1.036 & .003/.068/.946/1.052 \\
C-1011 & g-comp & 0/0/0 & -.002/.111/.946/1.265 & -.003/.087/.938/1.060 & -.001/.076/.932/.999 & .000/.058/.942/1.035 \\
\addlinespace[1.2pt]
C-1010 & Can-par & 1/0/0 & .003/.136/.950/1.168 & -.003/.102/.957/1.239 & .001/.088/.960/1.217 & .002/.068/.973/1.299 \\
C-1010 & Can-SL & 1/0/0 & .001/.141/.947/1.191 & -.001/.104/.957/1.247 & .001/.091/.964/1.227 & .003/.069/.975/1.322 \\
C-1010 & g-comp & 0/0/0 & -.002/.111/.946/1.265 & -.003/.087/.938/1.060 & -.001/.076/.932/.999 & .000/.058/.942/1.035 \\
\addlinespace[1.2pt]
C-1001 & Can-par & 0/0/0 & .066/.184/.927/.897 & .065/.146/.930/.912 & .062/.131/.916/.880 & .064/.110/.900/.920 \\
C-1001 & Can-SL & 0/0/0 & .065/.182/.944/.959 & .065/.145/.936/.947 & .060/.130/.920/.901 & .063/.109/.906/.938 \\
C-1001 & g-comp & 0/0/0 & .060/.169/.964/1.190 & .063/.139/.937/1.050 & .058/.122/.925/1.007 & .063/.106/.896/1.016 \\
\addlinespace[1.2pt]
C-1000 & Can-par & 0/0/0 & .065/.185/.941/.921 & .064/.145/.947/.966 & .061/.130/.935/.930 & .064/.110/.917/.976 \\
C-1000 & Can-SL & 0/0/0 & .067/.184/.947/.942 & .065/.144/.944/.974 & .060/.130/.933/.925 & .064/.110/.918/.976 \\
C-1000 & g-comp & 0/0/0 & .060/.169/.964/1.190 & .063/.139/.937/1.050 & .058/.122/.925/1.007 & .063/.106/.896/1.016 \\
\addlinespace[1.2pt]
C-0111 & Can-par & 1/0/0 & .003/.142/.929/1.017 & .001/.107/.936/1.015 & .002/.092/.936/1.016 & .002/.069/.946/1.049 \\
C-0111 & Can-SL & 1/0/0 & .008/.151/.945/1.157 & .006/.114/.943/1.097 & .005/.096/.949/1.075 & .005/.073/.950/1.092 \\
C-0111 & g-comp & 0/0/0 & .017/.112/.953/1.096 & .018/.090/.946/1.038 & .020/.081/.933/.977 & .021/.062/.946/1.049 \\
\addlinespace[1.2pt]
C-0110 & Can-par & 0/0/0 & .013/.138/.959/1.211 & .009/.107/.969/1.262 & .012/.093/.972/1.266 & .014/.072/.984/1.361 \\
C-0110 & Can-SL & 0/0/0 & .017/.147/.964/1.219 & .014/.113/.973/1.273 & .017/.099/.972/1.276 & .018/.076/.985/1.385 \\
C-0110 & g-comp & 0/0/0 & .017/.112/.953/1.096 & .018/.090/.946/1.038 & .020/.081/.933/.977 & .021/.062/.946/1.049 \\
\addlinespace[1.2pt]
C-0101 & Can-par & 0/0/0 & .104/.201/.947/.951 & .101/.168/.925/.967 & .095/.153/.897/.928 & .096/.133/.862/.991 \\
C-0101 & Can-SL & 0/0/0 & .108/.205/.949/1.010 & .104/.171/.931/.994 & .096/.154/.904/.946 & .096/.133/.868/1.005 \\
C-0101 & g-comp & 0/0/0 & .114/.200/.929/1.052 & .117/.176/.882/1.020 & .113/.161/.836/.986 & .118/.148/.738/1.031 \\
\addlinespace[1.2pt]
C-0100 & Can-par & 0/0/0 & .104/.203/.957/.973 & .104/.170/.945/1.016 & .098/.155/.917/.970 & .101/.137/.878/1.039 \\
C-0100 & Can-SL & 0/0/0 & .108/.207/.956/.986 & .107/.173/.944/1.019 & .100/.158/.914/.964 & .103/.138/.871/1.034 \\
C-0100 & g-comp & 0/0/0 & .114/.200/.929/1.052 & .117/.176/.882/1.020 & .113/.161/.836/.986 & .118/.148/.738/1.031 \\
\addlinespace[1.2pt]
C-0011 & Can-par & 1/0/0 & .003/.142/.929/1.017 & .001/.107/.936/1.015 & .002/.092/.936/1.016 & .002/.069/.946/1.049 \\
C-0011 & Can-SL & 1/0/0 & .008/.151/.945/1.158 & .006/.114/.942/1.097 & .005/.096/.949/1.076 & .005/.073/.950/1.091 \\
C-0011 & g-comp & 0/0/0 & .017/.112/.953/1.096 & .018/.090/.946/1.038 & .020/.081/.933/.977 & .021/.062/.946/1.049 \\
\addlinespace[1.2pt]
C-0010 & Can-par & 0/0/0 & .013/.138/.959/1.211 & .009/.107/.969/1.262 & .012/.093/.972/1.266 & .014/.072/.984/1.361 \\
C-0010 & Can-SL & 0/0/0 & .018/.147/.964/1.220 & .014/.113/.973/1.272 & .017/.099/.973/1.277 & .018/.076/.985/1.385 \\
C-0010 & g-comp & 0/0/0 & .017/.112/.953/1.096 & .018/.090/.946/1.038 & .020/.081/.933/.977 & .021/.062/.946/1.049 \\
\addlinespace[1.2pt]
C-0001 & Can-par & 0/0/0 & .104/.201/.947/.951 & .101/.168/.925/.967 & .095/.153/.897/.928 & .096/.133/.862/.991 \\
C-0001 & Can-SL & 0/0/0 & .108/.205/.950/1.011 & .104/.171/.931/.995 & .095/.153/.905/.948 & .096/.133/.869/1.005 \\
C-0001 & g-comp & 0/0/0 & .114/.200/.929/1.052 & .117/.176/.882/1.020 & .113/.161/.836/.986 & .118/.148/.738/1.031 \\
\addlinespace[1.2pt]
C-0000 & Can-par & 0/0/0 & .104/.203/.957/.973 & .104/.170/.945/1.016 & .098/.155/.917/.970 & .101/.137/.878/1.039 \\
C-0000 & Can-SL & 0/0/0 & .108/.207/.958/.987 & .106/.172/.944/1.020 & .100/.158/.915/.966 & .102/.138/.870/1.034 \\
C-0000 & g-comp & 0/0/0 & .114/.200/.929/1.052 & .117/.176/.882/1.020 & .113/.161/.836/.986 & .118/.148/.738/1.031 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Low-dimensional-study performance for the IDE, $W_i=N_i$.}\label{tab:sim-ld-IDE-I}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
LD-AC & G+glmnet & 1/1/1 & .004/.271/.948/1.067 & .004/.213/.951/1.044 & .007/.181/.957/1.031 & .003/.146/.954/1.038 \\
LD-AC & G+RF & 1/1/1 & .003/.276/.949/1.071 & .004/.218/.954/1.041 & .006/.181/.960/1.051 & .001/.145/.952/1.046 \\
LD-AC & G+SL & 1/1/1 & .000/.279/.968/1.338 & .005/.224/.960/1.144 & .006/.186/.965/1.101 & .003/.147/.962/1.086 \\
LD-AC & RB+glmnet & 1/1/1 & .004/.271/.946/1.065 & .005/.213/.949/1.042 & .006/.181/.959/1.038 & .003/.146/.954/1.043 \\
LD-AC & RB+RF & 1/1/1 & .003/.277/.948/1.065 & .003/.217/.951/1.045 & .006/.181/.961/1.051 & .002/.145/.955/1.046 \\
LD-AC & RB+SL & 1/1/1 & .001/.282/.968/1.319 & .003/.227/.956/1.126 & .006/.185/.966/1.107 & .003/.147/.959/1.086 \\
\addlinespace[1.2pt]
LD-T2 & G+glmnet & 1/0/0 & .003/.269/.947/1.043 & .007/.209/.952/1.019 & .006/.179/.954/.997 & .003/.142/.952/1.009 \\
LD-T2 & G+RF & 1/0/0 & .000/.285/.952/1.083 & .002/.228/.959/1.095 & .005/.197/.968/1.122 & .003/.161/.978/1.208 \\
LD-T2 & G+SL & 1/0/0 & .000/.280/.975/1.436 & .007/.223/.985/1.613 & .003/.188/.993/1.654 & .003/.148/.983/1.406 \\
LD-T2 & RB+glmnet & 1/0/0 & .004/.268/.945/1.047 & .007/.209/.948/1.019 & .007/.179/.949/.996 & .002/.142/.955/1.009 \\
LD-T2 & RB+RF & 1/0/0 & -.001/.285/.946/1.086 & .003/.229/.960/1.092 & .006/.196/.975/1.126 & .003/.160/.978/1.209 \\
LD-T2 & RB+SL & 1/0/0 & -.002/.285/.978/1.430 & .006/.223/.983/1.614 & .006/.187/.986/1.664 & .003/.146/.984/1.428 \\
\addlinespace[1.2pt]
LD-T3 & G+glmnet & 1/0/0 & .021/.275/.955/1.083 & .016/.218/.951/1.056 & .019/.188/.956/1.036 & .014/.151/.951/1.046 \\
LD-T3 & G+RF & 1/0/0 & .020/.279/.954/1.084 & .017/.221/.952/1.061 & .018/.188/.963/1.057 & .011/.149/.955/1.055 \\
LD-T3 & G+SL & 1/0/0 & .016/.283/.963/1.344 & .014/.231/.962/1.151 & .016/.191/.967/1.120 & .010/.151/.960/1.100 \\
LD-T3 & RB+glmnet & 1/0/0 & .021/.275/.954/1.078 & .016/.219/.949/1.049 & .019/.186/.959/1.046 & .014/.151/.952/1.053 \\
LD-T3 & RB+RF & 1/0/0 & .021/.280/.952/1.080 & .015/.221/.952/1.059 & .018/.188/.962/1.054 & .012/.150/.955/1.051 \\
LD-T3 & RB+SL & 1/0/0 & .018/.284/.968/1.335 & .011/.233/.959/1.136 & .017/.191/.969/1.122 & .010/.152/.957/1.099 \\
\addlinespace[1.2pt]
LD-T4 & G+glmnet & 0/0/0 & .009/.270/.952/1.040 & .007/.210/.950/1.026 & .010/.183/.948/.995 & .005/.147/.948/1.017 \\
LD-T4 & G+RF & 0/0/0 & .009/.274/.955/1.043 & .006/.214/.951/1.031 & .009/.184/.955/1.011 & .003/.145/.950/1.020 \\
LD-T4 & G+SL & 0/0/0 & .005/.277/.967/1.317 & .004/.223/.962/1.134 & .009/.188/.959/1.070 & .003/.148/.957/1.064 \\
LD-T4 & RB+glmnet & 0/0/0 & .010/.269/.953/1.037 & .006/.211/.952/1.019 & .009/.183/.950/1.001 & .004/.147/.949/1.024 \\
LD-T4 & RB+RF & 0/0/0 & .009/.275/.957/1.040 & .005/.214/.951/1.029 & .009/.184/.952/1.011 & .004/.146/.951/1.020 \\
LD-T4 & RB+SL & 0/0/0 & .007/.280/.972/1.304 & .001/.226/.957/1.119 & .009/.187/.965/1.075 & .003/.149/.954/1.060 \\
\addlinespace[1.2pt]
LD-T5 & G+glmnet & 0/0/0 & .019/.275/.956/1.083 & .017/.219/.951/1.052 & .018/.186/.958/1.041 & .013/.149/.950/1.038 \\
LD-T5 & G+RF & 0/0/0 & .014/.288/.951/1.130 & .010/.236/.961/1.138 & .015/.207/.973/1.155 & .015/.168/.982/1.241 \\
LD-T5 & G+SL & 0/0/0 & .014/.284/.974/1.478 & .014/.233/.988/1.648 & .015/.197/.992/1.718 & .012/.155/.984/1.473 \\
LD-T5 & RB+glmnet & 0/0/0 & .020/.274/.954/1.086 & .015/.218/.947/1.054 & .018/.187/.956/1.039 & .013/.148/.951/1.046 \\
LD-T5 & RB+RF & 0/0/0 & .015/.287/.953/1.126 & .010/.237/.964/1.131 & .018/.207/.969/1.153 & .015/.169/.981/1.233 \\
LD-T5 & RB+SL & 0/0/0 & .015/.287/.977/1.469 & .011/.232/.985/1.661 & .016/.195/.988/1.739 & .012/.154/.990/1.482 \\
\addlinespace[1.2pt]
LD-T6 & G+glmnet & 0/0/0 & .008/.270/.955/1.040 & .006/.211/.950/1.021 & .008/.182/.950/.998 & .004/.146/.950/1.008 \\
LD-T6 & G+RF & 0/0/0 & .004/.285/.955/1.087 & .000/.232/.961/1.101 & .006/.203/.971/1.122 & .005/.165/.977/1.211 \\
LD-T6 & G+SL & 0/0/0 & .004/.280/.977/1.434 & .005/.228/.987/1.626 & .005/.193/.991/1.688 & .003/.152/.982/1.433 \\
LD-T6 & RB+glmnet & 0/0/0 & .008/.269/.954/1.043 & .005/.210/.946/1.025 & .009/.183/.948/.994 & .004/.145/.951/1.014 \\
LD-T6 & RB+RF & 0/0/0 & .004/.283/.958/1.092 & .001/.233/.960/1.095 & .008/.202/.964/1.119 & .005/.166/.976/1.201 \\
LD-T6 & RB+SL & 0/0/0 & .004/.283/.977/1.433 & .001/.226/.985/1.639 & .006/.192/.987/1.699 & .002/.151/.988/1.453 \\
\addlinespace[1.2pt]
LD-U2 & G+glmnet & 1/0/0 & .004/.271/.948/1.067 & .004/.213/.951/1.044 & .007/.181/.957/1.031 & .003/.146/.954/1.038 \\
LD-U2 & G+RF & 1/0/0 & .003/.276/.949/1.071 & .004/.218/.954/1.041 & .006/.181/.960/1.051 & .001/.145/.952/1.046 \\
LD-U2 & G+SL & 1/0/0 & .000/.279/.968/1.338 & .005/.224/.960/1.144 & .006/.186/.965/1.101 & .003/.147/.962/1.086 \\
LD-U2 & RB+glmnet & 1/0/0 & .004/.271/.946/1.065 & .005/.213/.949/1.042 & .006/.181/.959/1.038 & .003/.146/.954/1.043 \\
LD-U2 & RB+RF & 1/0/0 & .003/.277/.948/1.065 & .003/.217/.951/1.045 & .006/.181/.961/1.051 & .002/.145/.955/1.046 \\
LD-U2 & RB+SL & 1/0/0 & .001/.282/.968/1.319 & .003/.227/.956/1.126 & .006/.185/.966/1.107 & .003/.147/.959/1.086 \\
\addlinespace[1.2pt]
LD-U3 & G+glmnet & 1/0/0 & .004/.271/.948/1.067 & .004/.213/.951/1.044 & .007/.181/.957/1.031 & .003/.146/.954/1.038 \\
LD-U3 & G+RF & 1/0/0 & .003/.276/.949/1.071 & .004/.218/.954/1.041 & .006/.181/.960/1.051 & .001/.145/.952/1.046 \\
LD-U3 & G+SL & 1/0/0 & .000/.279/.968/1.338 & .005/.224/.960/1.144 & .006/.186/.965/1.101 & .003/.147/.962/1.086 \\
LD-U3 & RB+glmnet & 1/0/0 & .004/.271/.946/1.065 & .005/.213/.949/1.042 & .006/.181/.959/1.038 & .003/.146/.954/1.043 \\
LD-U3 & RB+RF & 1/0/0 & .003/.277/.948/1.065 & .003/.217/.951/1.045 & .006/.181/.961/1.051 & .002/.145/.955/1.046 \\
LD-U3 & RB+SL & 1/0/0 & .001/.282/.968/1.319 & .003/.227/.956/1.126 & .006/.185/.966/1.107 & .003/.147/.959/1.086 \\
\addlinespace[1.2pt]
LD-U4 & G+glmnet & 1/0/0 & .004/.271/.948/1.067 & .004/.213/.951/1.044 & .007/.181/.957/1.031 & .003/.146/.954/1.038 \\
LD-U4 & G+RF & 1/0/0 & .003/.276/.949/1.071 & .004/.218/.954/1.041 & .006/.181/.960/1.051 & .001/.145/.952/1.046 \\
LD-U4 & G+SL & 1/0/0 & .000/.279/.968/1.338 & .005/.224/.960/1.144 & .006/.186/.965/1.101 & .003/.147/.962/1.086 \\
LD-U4 & RB+glmnet & 1/0/0 & .004/.271/.946/1.065 & .005/.213/.949/1.042 & .006/.181/.959/1.038 & .003/.146/.954/1.043 \\
LD-U4 & RB+RF & 1/0/0 & .003/.277/.948/1.065 & .003/.217/.951/1.045 & .006/.181/.961/1.051 & .002/.145/.955/1.046 \\
LD-U4 & RB+SL & 1/0/0 & .001/.282/.968/1.319 & .003/.227/.956/1.126 & .006/.185/.966/1.107 & .003/.147/.959/1.086 \\
\addlinespace[1.2pt]
LD-U5 & G+glmnet & 1/0/0 & .004/.271/.948/1.067 & .004/.213/.951/1.044 & .007/.181/.957/1.031 & .003/.146/.954/1.038 \\
LD-U5 & G+RF & 1/0/0 & .003/.276/.949/1.071 & .004/.218/.954/1.041 & .006/.181/.960/1.051 & .001/.145/.952/1.046 \\
LD-U5 & G+SL & 1/0/0 & .000/.279/.968/1.338 & .005/.224/.960/1.144 & .006/.186/.965/1.101 & .003/.147/.962/1.086 \\
LD-U5 & RB+glmnet & 1/0/0 & .004/.271/.946/1.065 & .005/.213/.949/1.042 & .006/.181/.959/1.038 & .003/.146/.954/1.043 \\
LD-U5 & RB+RF & 1/0/0 & .003/.277/.948/1.065 & .003/.217/.951/1.045 & .006/.181/.961/1.051 & .002/.145/.955/1.046 \\
LD-U5 & RB+SL & 1/0/0 & .001/.282/.968/1.319 & .003/.227/.956/1.126 & .006/.185/.966/1.107 & .003/.147/.959/1.086 \\
\addlinespace[1.2pt]
LD-U6 & G+glmnet & 1/0/0 & .004/.271/.948/1.067 & .004/.213/.951/1.044 & .007/.181/.957/1.031 & .003/.146/.954/1.038 \\
LD-U6 & G+RF & 1/0/0 & .003/.276/.949/1.071 & .004/.218/.954/1.041 & .006/.181/.960/1.051 & .001/.145/.952/1.046 \\
LD-U6 & G+SL & 1/0/0 & .000/.279/.968/1.338 & .005/.224/.960/1.144 & .006/.186/.965/1.101 & .003/.147/.962/1.086 \\
LD-U6 & RB+glmnet & 1/0/0 & .004/.271/.946/1.065 & .005/.213/.949/1.042 & .006/.181/.959/1.038 & .003/.146/.954/1.043 \\
LD-U6 & RB+RF & 1/0/0 & .003/.277/.948/1.065 & .003/.217/.951/1.045 & .006/.181/.961/1.051 & .002/.145/.955/1.046 \\
LD-U6 & RB+SL & 1/0/0 & .001/.282/.968/1.319 & .003/.227/.956/1.126 & .006/.185/.966/1.107 & .003/.147/.959/1.086 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Low-dimensional-study performance for the IIME, $W_i=N_i$.}\label{tab:sim-ld-IIME-I}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
LD-AC & G+glmnet & 1/1/1 & -.005/.243/.964/1.059 & -.003/.196/.960/1.000 & -.008/.166/.953/1.001 & -.001/.131/.959/1.020 \\
LD-AC & G+RF & 1/1/1 & -.005/.243/.964/1.058 & -.004/.196/.958/1.000 & -.008/.166/.954/1.001 & -.001/.131/.961/1.021 \\
LD-AC & G+SL & 1/1/1 & -.006/.242/.967/1.068 & -.003/.196/.960/1.005 & -.008/.166/.952/1.003 & -.001/.131/.960/1.023 \\
LD-AC & RB+glmnet & 1/1/1 & -.005/.243/.962/1.059 & -.004/.196/.958/1.000 & -.008/.166/.954/1.001 & -.001/.131/.959/1.020 \\
LD-AC & RB+RF & 1/1/1 & -.005/.243/.966/1.059 & -.003/.196/.959/1.000 & -.008/.166/.954/1.004 & -.001/.131/.959/1.020 \\
LD-AC & RB+SL & 1/1/1 & -.005/.243/.966/1.063 & -.003/.196/.961/1.007 & -.008/.166/.955/1.008 & -.001/.131/.959/1.022 \\
\addlinespace[1.2pt]
LD-T2 & G+glmnet & 1/0/0 & -.005/.254/.965/1.130 & -.006/.201/.966/1.056 & -.007/.170/.959/1.039 & -.001/.135/.964/1.049 \\
LD-T2 & G+RF & 1/0/0 & -.005/.259/.966/1.156 & -.004/.209/.968/1.086 & -.007/.178/.968/1.087 & -.002/.143/.974/1.121 \\
LD-T2 & G+SL & 1/0/0 & -.005/.263/.978/1.356 & -.005/.209/.979/1.369 & -.005/.177/.981/1.365 & -.001/.137/.983/1.236 \\
LD-T2 & RB+glmnet & 1/0/0 & -.005/.255/.965/1.128 & -.006/.202/.965/1.054 & -.009/.170/.961/1.042 & -.001/.134/.962/1.059 \\
LD-T2 & RB+RF & 1/0/0 & -.004/.259/.968/1.156 & -.006/.210/.967/1.083 & -.007/.178/.966/1.085 & -.001/.145/.970/1.108 \\
LD-T2 & RB+SL & 1/0/0 & -.005/.263/.978/1.377 & -.006/.211/.982/1.357 & -.008/.176/.980/1.366 & -.000/.138/.976/1.236 \\
\addlinespace[1.2pt]
LD-T3 & G+glmnet & 1/0/0 & -.011/.261/.966/1.099 & -.006/.205/.963/1.025 & -.011/.172/.958/1.030 & -.006/.135/.961/1.044 \\
LD-T3 & G+RF & 1/0/0 & -.012/.262/.965/1.098 & -.007/.206/.961/1.026 & -.010/.174/.957/1.026 & -.002/.134/.961/1.046 \\
LD-T3 & G+SL & 1/0/0 & -.012/.262/.969/1.146 & -.008/.208/.963/1.056 & -.012/.174/.961/1.049 & -.005/.136/.963/1.049 \\
LD-T3 & RB+glmnet & 1/0/0 & -.011/.261/.967/1.097 & -.007/.205/.960/1.026 & -.012/.173/.958/1.028 & -.006/.135/.963/1.044 \\
LD-T3 & RB+RF & 1/0/0 & -.011/.261/.967/1.102 & -.007/.206/.962/1.026 & -.011/.173/.964/1.033 & -.003/.135/.962/1.046 \\
LD-T3 & RB+SL & 1/0/0 & -.012/.261/.968/1.162 & -.008/.209/.965/1.049 & -.012/.174/.960/1.052 & -.005/.136/.962/1.048 \\
\addlinespace[1.2pt]
LD-T4 & G+glmnet & 0/0/0 & .000/.268/.968/1.128 & .003/.210/.963/1.048 & -.002/.174/.958/1.048 & .003/.137/.963/1.058 \\
LD-T4 & G+RF & 0/0/0 & -.001/.269/.966/1.126 & .003/.211/.962/1.048 & -.002/.176/.958/1.046 & .006/.136/.963/1.066 \\
LD-T4 & G+SL & 0/0/0 & -.001/.268/.968/1.184 & .002/.213/.966/1.086 & -.004/.177/.963/1.069 & .001/.138/.962/1.067 \\
LD-T4 & RB+glmnet & 0/0/0 & .000/.268/.966/1.124 & .004/.210/.961/1.046 & -.003/.175/.959/1.047 & .003/.136/.963/1.065 \\
LD-T4 & RB+RF & 0/0/0 & .001/.267/.970/1.133 & .003/.212/.961/1.046 & -.002/.176/.962/1.049 & .005/.136/.960/1.066 \\
LD-T4 & RB+SL & 0/0/0 & -.001/.268/.969/1.197 & .001/.214/.966/1.072 & -.005/.176/.959/1.071 & .002/.138/.963/1.068 \\
\addlinespace[1.2pt]
LD-T5 & G+glmnet & 0/0/0 & -.011/.261/.966/1.104 & -.008/.206/.962/1.032 & -.011/.174/.957/1.032 & -.009/.138/.960/1.043 \\
LD-T5 & G+RF & 0/0/0 & -.010/.266/.969/1.151 & -.006/.217/.967/1.074 & -.013/.182/.969/1.106 & -.010/.146/.977/1.149 \\
LD-T5 & G+SL & 0/0/0 & -.013/.269/.978/1.367 & -.014/.216/.979/1.392 & -.022/.183/.983/1.418 & -.024/.143/.983/1.263 \\
LD-T5 & RB+glmnet & 0/0/0 & -.011/.262/.966/1.101 & -.007/.207/.960/1.027 & -.014/.175/.961/1.034 & -.010/.137/.965/1.051 \\
LD-T5 & RB+RF & 0/0/0 & -.010/.266/.968/1.138 & -.007/.217/.966/1.072 & -.014/.183/.968/1.099 & -.009/.147/.975/1.142 \\
LD-T5 & RB+SL & 0/0/0 & -.014/.269/.986/1.388 & -.014/.218/.980/1.383 & -.024/.183/.983/1.421 & -.023/.143/.976/1.267 \\
\addlinespace[1.2pt]
LD-T6 & G+glmnet & 0/0/0 & .000/.268/.967/1.131 & .002/.211/.964/1.050 & -.002/.176/.958/1.046 & -.000/.139/.964/1.060 \\
LD-T6 & G+RF & 0/0/0 & .001/.273/.971/1.161 & .004/.222/.964/1.075 & -.004/.185/.968/1.108 & -.000/.147/.977/1.146 \\
LD-T6 & G+SL & 0/0/0 & -.003/.277/.978/1.357 & -.005/.221/.979/1.379 & -.013/.184/.983/1.412 & -.014/.143/.984/1.265 \\
LD-T6 & RB+glmnet & 0/0/0 & .000/.270/.969/1.124 & .003/.212/.962/1.047 & -.004/.177/.960/1.046 & -.001/.138/.967/1.068 \\
LD-T6 & RB+RF & 0/0/0 & .001/.273/.970/1.155 & .002/.221/.964/1.076 & -.004/.185/.969/1.100 & .001/.148/.976/1.136 \\
LD-T6 & RB+SL & 0/0/0 & -.003/.276/.982/1.384 & -.005/.222/.983/1.368 & -.014/.185/.982/1.409 & -.013/.144/.980/1.269 \\
\addlinespace[1.2pt]
LD-U2 & G+glmnet & 1/0/0 & -.007/.248/.972/1.117 & -.001/.201/.965/1.041 & -.011/.170/.959/1.037 & -.002/.135/.964/1.051 \\
LD-U2 & G+RF & 1/0/0 & -.007/.255/.976/1.135 & -.004/.209/.964/1.072 & -.010/.181/.964/1.072 & -.001/.145/.962/1.105 \\
LD-U2 & G+SL & 1/0/0 & -.007/.256/.984/1.371 & -.003/.214/.980/1.320 & -.012/.176/.982/1.367 & -.002/.139/.977/1.227 \\
LD-U2 & RB+glmnet & 1/0/0 & -.006/.248/.971/1.120 & -.002/.200/.967/1.045 & -.009/.170/.962/1.038 & -.002/.136/.962/1.045 \\
LD-U2 & RB+RF & 1/0/0 & -.006/.255/.976/1.134 & -.002/.209/.966/1.074 & -.011/.180/.968/1.073 & -.002/.143/.962/1.115 \\
LD-U2 & RB+SL & 1/0/0 & -.006/.258/.987/1.371 & -.002/.211/.979/1.342 & -.010/.177/.976/1.351 & -.003/.138/.977/1.233 \\
\addlinespace[1.2pt]
LD-U3 & G+glmnet & 1/0/0 & -.005/.250/.969/1.124 & -.003/.198/.964/1.028 & -.007/.168/.952/1.006 & .002/.133/.955/1.011 \\
LD-U3 & G+RF & 1/0/0 & -.006/.251/.966/1.125 & -.003/.198/.964/1.033 & -.008/.168/.953/1.018 & -.002/.133/.955/1.010 \\
LD-U3 & G+SL & 1/0/0 & -.007/.251/.970/1.177 & -.002/.200/.964/1.061 & -.006/.169/.955/1.033 & .001/.132/.957/1.034 \\
LD-U3 & RB+glmnet & 1/0/0 & -.005/.251/.969/1.118 & -.003/.198/.961/1.025 & -.007/.168/.954/1.011 & .001/.133/.952/1.011 \\
LD-U3 & RB+RF & 1/0/0 & -.005/.251/.968/1.123 & -.003/.198/.961/1.032 & -.008/.168/.955/1.019 & -.001/.133/.955/1.009 \\
LD-U3 & RB+SL & 1/0/0 & -.007/.252/.969/1.186 & -.002/.199/.965/1.069 & -.006/.169/.957/1.039 & .000/.132/.961/1.030 \\
\addlinespace[1.2pt]
LD-U4 & G+glmnet & 0/0/0 & -.023/.254/.968/1.125 & -.019/.200/.961/1.052 & -.025/.172/.955/1.025 & -.015/.136/.957/1.025 \\
LD-U4 & G+RF & 0/0/0 & -.022/.254/.967/1.124 & -.020/.201/.964/1.058 & -.024/.172/.957/1.032 & -.017/.137/.957/1.021 \\
LD-U4 & G+SL & 0/0/0 & -.023/.255/.969/1.183 & -.018/.203/.967/1.091 & -.022/.173/.959/1.053 & -.013/.136/.961/1.043 \\
LD-U4 & RB+glmnet & 0/0/0 & -.023/.255/.967/1.118 & -.020/.201/.962/1.047 & -.024/.171/.955/1.031 & -.015/.136/.956/1.022 \\
LD-U4 & RB+RF & 0/0/0 & -.023/.256/.967/1.119 & -.019/.201/.963/1.059 & -.025/.172/.957/1.034 & -.017/.137/.960/1.023 \\
LD-U4 & RB+SL & 0/0/0 & -.022/.257/.968/1.189 & -.017/.201/.969/1.096 & -.022/.173/.958/1.052 & -.014/.136/.962/1.042 \\
\addlinespace[1.2pt]
LD-U5 & G+glmnet & 0/0/0 & -.005/.251/.969/1.123 & -.001/.199/.961/1.028 & -.007/.170/.954/1.012 & .005/.136/.959/1.016 \\
LD-U5 & G+RF & 0/0/0 & -.008/.260/.970/1.145 & -.006/.208/.967/1.093 & -.008/.183/.960/1.070 & .003/.147/.961/1.093 \\
LD-U5 & G+SL & 0/0/0 & -.006/.260/.981/1.418 & .002/.212/.985/1.393 & .001/.176/.983/1.423 & .017/.140/.977/1.253 \\
LD-U5 & RB+glmnet & 0/0/0 & -.005/.251/.968/1.125 & -.002/.198/.962/1.035 & -.004/.170/.953/1.016 & .005/.136/.958/1.012 \\
LD-U5 & RB+RF & 0/0/0 & -.007/.259/.969/1.145 & -.004/.207/.971/1.095 & -.007/.183/.960/1.067 & .002/.145/.965/1.110 \\
LD-U5 & RB+SL & 0/0/0 & -.005/.263/.980/1.412 & .002/.208/.983/1.418 & .003/.177/.977/1.419 & .016/.140/.976/1.252 \\
\addlinespace[1.2pt]
LD-U6 & G+glmnet & 0/0/0 & -.023/.255/.967/1.125 & -.018/.202/.959/1.049 & -.024/.173/.957/1.032 & -.011/.138/.954/1.026 \\
LD-U6 & G+RF & 0/0/0 & -.024/.264/.968/1.138 & -.021/.210/.963/1.088 & -.023/.185/.955/1.076 & -.012/.148/.959/1.093 \\
LD-U6 & G+SL & 0/0/0 & -.021/.263/.980/1.382 & -.012/.214/.983/1.373 & -.015/.178/.982/1.415 & .002/.140/.976/1.244 \\
LD-U6 & RB+glmnet & 0/0/0 & -.023/.255/.967/1.124 & -.019/.201/.964/1.055 & -.022/.173/.955/1.034 & -.011/.138/.955/1.023 \\
LD-U6 & RB+RF & 0/0/0 & -.023/.263/.965/1.138 & -.019/.210/.965/1.092 & -.023/.184/.965/1.075 & -.013/.146/.966/1.109 \\
LD-U6 & RB+SL & 0/0/0 & -.020/.266/.980/1.379 & -.013/.210/.979/1.394 & -.013/.179/.980/1.399 & .000/.140/.977/1.245 \\
\bottomrule
\end{longtable}
}
\end{landscape}

\begin{landscape}
{\tiny
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{0.88}
\begin{longtable}{@{}llc*{4}{c}@{}}
\caption{Low-dimensional-study performance for the ISME, $W_i=N_i$.}\label{tab:sim-ld-ISME-I}\\
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endfirsthead
\toprule
Scenario & Method & P/AL/CI & $K=50$ & $K=75$ & $K=100$ & $K=150$ \\
\midrule
\endhead
LD-AC & G+glmnet & 1/1/1 & .001/.149/.956/1.326 & -.000/.108/.957/1.180 & -.001/.092/.946/1.085 & .000/.069/.956/1.073 \\
LD-AC & G+RF & 1/1/1 & .001/.149/.954/1.333 & -.000/.108/.956/1.202 & -.001/.092/.951/1.105 & .001/.069/.951/1.078 \\
LD-AC & G+SL & 1/1/1 & .002/.149/.960/1.438 & -.001/.109/.960/1.255 & -.001/.092/.949/1.162 & .001/.070/.946/1.111 \\
LD-AC & RB+glmnet & 1/1/1 & .001/.149/.954/1.319 & -.001/.109/.957/1.181 & -.001/.091/.949/1.095 & .001/.069/.951/1.075 \\
LD-AC & RB+RF & 1/1/1 & .000/.149/.954/1.328 & -.000/.110/.959/1.189 & -.001/.092/.949/1.107 & .001/.069/.953/1.085 \\
LD-AC & RB+SL & 1/1/1 & .001/.150/.957/1.421 & -.001/.111/.955/1.225 & -.001/.092/.950/1.156 & .001/.069/.952/1.124 \\
\addlinespace[1.2pt]
LD-T2 & G+glmnet & 1/0/0 & -.000/.150/.953/1.323 & .000/.110/.956/1.178 & -.003/.094/.944/1.083 & .001/.073/.951/1.058 \\
LD-T2 & G+RF & 1/0/0 & .000/.163/.963/1.314 & -.002/.127/.965/1.196 & -.001/.112/.961/1.140 & .002/.090/.968/1.179 \\
LD-T2 & G+SL & 1/0/0 & .001/.165/.978/1.689 & -.001/.130/.982/1.673 & -.004/.105/.977/1.678 & .002/.078/.974/1.423 \\
LD-T2 & RB+glmnet & 1/0/0 & .001/.149/.953/1.326 & .000/.110/.957/1.179 & -.001/.094/.946/1.083 & .001/.073/.950/1.064 \\
LD-T2 & RB+RF & 1/0/0 & -.000/.165/.956/1.293 & -.001/.128/.964/1.185 & -.002/.112/.965/1.137 & .001/.088/.975/1.192 \\
LD-T2 & RB+SL & 1/0/0 & .000/.168/.978/1.692 & .000/.129/.981/1.693 & -.002/.106/.978/1.659 & .001/.078/.977/1.424 \\
\addlinespace[1.2pt]
LD-T3 & G+glmnet & 1/0/0 & -.009/.156/.954/1.321 & -.009/.112/.956/1.187 & -.010/.097/.938/1.080 & -.006/.073/.951/1.080 \\
LD-T3 & G+RF & 1/0/0 & -.008/.157/.949/1.322 & -.010/.113/.956/1.199 & -.010/.097/.944/1.101 & -.009/.073/.954/1.079 \\
LD-T3 & G+SL & 1/0/0 & -.008/.159/.959/1.461 & -.008/.117/.963/1.281 & -.008/.099/.945/1.159 & -.004/.073/.950/1.130 \\
LD-T3 & RB+glmnet & 1/0/0 & -.009/.156/.949/1.307 & -.010/.113/.955/1.183 & -.009/.096/.941/1.091 & -.005/.072/.952/1.085 \\
LD-T3 & RB+RF & 1/0/0 & -.009/.158/.954/1.311 & -.009/.115/.958/1.190 & -.009/.097/.944/1.096 & -.009/.073/.948/1.085 \\
LD-T3 & RB+SL & 1/0/0 & -.007/.160/.957/1.480 & -.006/.119/.959/1.255 & -.007/.099/.949/1.153 & -.005/.073/.951/1.132 \\
\addlinespace[1.2pt]
LD-T4 & G+glmnet & 1/0/0 & -.009/.156/.954/1.321 & -.009/.112/.956/1.187 & -.010/.097/.938/1.080 & -.006/.073/.951/1.080 \\
LD-T4 & G+RF & 1/0/0 & -.008/.157/.949/1.322 & -.010/.113/.956/1.199 & -.010/.097/.944/1.101 & -.009/.073/.954/1.079 \\
LD-T4 & G+SL & 1/0/0 & -.008/.159/.959/1.461 & -.008/.117/.963/1.281 & -.008/.099/.945/1.159 & -.004/.073/.950/1.130 \\
LD-T4 & RB+glmnet & 1/0/0 & -.009/.156/.949/1.307 & -.010/.113/.955/1.183 & -.009/.096/.941/1.091 & -.005/.072/.952/1.085 \\
LD-T4 & RB+RF & 1/0/0 & -.009/.158/.954/1.311 & -.009/.115/.958/1.190 & -.009/.097/.944/1.096 & -.009/.073/.948/1.085 \\
LD-T4 & RB+SL & 1/0/0 & -.007/.160/.957/1.480 & -.006/.119/.959/1.255 & -.007/.099/.949/1.153 & -.005/.073/.951/1.132 \\
\addlinespace[1.2pt]
LD-T5 & G+glmnet & 0/0/0 & -.009/.157/.953/1.313 & -.008/.114/.955/1.177 & -.010/.098/.935/1.078 & -.002/.077/.947/1.049 \\
LD-T5 & G+RF & 0/0/0 & -.008/.172/.959/1.295 & -.009/.134/.965/1.184 & -.007/.119/.954/1.132 & -.002/.095/.970/1.190 \\
LD-T5 & G+SL & 0/0/0 & -.004/.173/.976/1.669 & .000/.135/.985/1.689 & .003/.111/.982/1.712 & .013/.084/.980/1.441 \\
LD-T5 & RB+glmnet & 0/0/0 & -.009/.157/.951/1.311 & -.008/.114/.958/1.184 & -.007/.099/.939/1.077 & -.002/.077/.948/1.053 \\
LD-T5 & RB+RF & 0/0/0 & -.010/.174/.955/1.280 & -.008/.134/.970/1.189 & -.007/.118/.961/1.131 & -.003/.093/.973/1.207 \\
LD-T5 & RB+SL & 0/0/0 & -.005/.177/.977/1.678 & .000/.133/.984/1.716 & .005/.113/.979/1.688 & .012/.084/.980/1.444 \\
\addlinespace[1.2pt]
LD-T6 & G+glmnet & 0/0/0 & -.009/.157/.953/1.313 & -.008/.114/.955/1.177 & -.010/.098/.935/1.078 & -.002/.077/.947/1.049 \\
LD-T6 & G+RF & 0/0/0 & -.008/.172/.959/1.295 & -.009/.134/.965/1.184 & -.007/.119/.954/1.132 & -.002/.095/.970/1.190 \\
LD-T6 & G+SL & 0/0/0 & -.004/.173/.976/1.669 & .000/.135/.985/1.689 & .003/.111/.982/1.712 & .013/.084/.980/1.441 \\
LD-T6 & RB+glmnet & 0/0/0 & -.009/.157/.951/1.311 & -.008/.114/.958/1.184 & -.007/.099/.939/1.077 & -.002/.077/.948/1.053 \\
LD-T6 & RB+RF & 0/0/0 & -.010/.174/.955/1.280 & -.008/.134/.970/1.189 & -.007/.118/.961/1.131 & -.003/.093/.973/1.207 \\
LD-T6 & RB+SL & 0/0/0 & -.005/.177/.977/1.678 & .000/.133/.984/1.716 & .005/.113/.979/1.688 & .012/.084/.980/1.444 \\
\addlinespace[1.2pt]
LD-U2 & G+glmnet & 1/0/0 & .003/.139/.951/1.172 & -.002/.103/.943/1.053 & .001/.088/.928/.982 & .001/.067/.940/1.008 \\
LD-U2 & G+RF & 1/0/0 & .003/.150/.951/1.203 & .000/.116/.958/1.147 & .001/.102/.961/1.138 & .001/.083/.970/1.215 \\
LD-U2 & G+SL & 1/0/0 & .003/.160/.975/1.692 & -.002/.119/.978/1.819 & .003/.098/.975/1.848 & .002/.073/.980/1.531 \\
LD-U2 & RB+glmnet & 1/0/0 & .002/.141/.948/1.170 & -.002/.103/.947/1.057 & -.000/.088/.931/.987 & .002/.068/.941/1.006 \\
LD-U2 & RB+RF & 1/0/0 & .001/.149/.953/1.206 & -.001/.117/.955/1.138 & .001/.103/.960/1.125 & .001/.084/.970/1.200 \\
LD-U2 & RB+SL & 1/0/0 & .002/.159/.972/1.715 & -.002/.122/.981/1.777 & .000/.098/.982/1.845 & .002/.072/.983/1.558 \\
\addlinespace[1.2pt]
LD-U3 & G+glmnet & 1/0/0 & .001/.158/.972/1.375 & -.001/.118/.965/1.212 & -.003/.100/.964/1.132 & -.002/.076/.965/1.121 \\
LD-U3 & G+RF & 1/0/0 & .001/.159/.973/1.377 & -.001/.120/.968/1.220 & -.001/.102/.966/1.147 & .002/.076/.961/1.132 \\
LD-U3 & G+SL & 1/0/0 & .003/.161/.973/1.521 & -.003/.123/.964/1.289 & -.003/.102/.963/1.223 & -.001/.077/.957/1.160 \\
LD-U3 & RB+glmnet & 1/0/0 & .001/.158/.970/1.364 & -.001/.118/.968/1.212 & -.002/.100/.965/1.138 & -.001/.076/.965/1.121 \\
LD-U3 & RB+RF & 1/0/0 & .000/.159/.971/1.373 & -.001/.120/.970/1.217 & -.002/.101/.968/1.159 & .001/.075/.965/1.138 \\
LD-U3 & RB+SL & 1/0/0 & .002/.162/.976/1.528 & -.002/.126/.968/1.268 & -.003/.102/.966/1.224 & -.001/.076/.963/1.179 \\
\addlinespace[1.2pt]
LD-U4 & G+glmnet & 0/0/0 & .019/.148/.961/1.196 & .016/.111/.958/1.088 & .015/.094/.952/1.027 & .014/.071/.956/1.052 \\
LD-U4 & G+RF & 0/0/0 & .018/.149/.965/1.198 & .016/.112/.962/1.097 & .015/.096/.953/1.033 & .017/.071/.960/1.063 \\
LD-U4 & G+SL & 0/0/0 & .020/.152/.963/1.352 & .013/.114/.961/1.195 & .013/.097/.952/1.095 & .013/.072/.953/1.088 \\
LD-U4 & RB+glmnet & 0/0/0 & .019/.148/.963/1.188 & .016/.111/.958/1.084 & .015/.095/.949/1.025 & .015/.071/.955/1.060 \\
LD-U4 & RB+RF & 0/0/0 & .018/.149/.964/1.202 & .016/.113/.964/1.090 & .015/.095/.953/1.043 & .016/.071/.959/1.064 \\
LD-U4 & RB+SL & 0/0/0 & .018/.151/.966/1.385 & .013/.117/.962/1.168 & .012/.096/.955/1.097 & .013/.072/.956/1.092 \\
\addlinespace[1.2pt]
LD-U5 & G+glmnet & 0/0/0 & .001/.158/.971/1.378 & -.002/.119/.969/1.210 & -.003/.101/.967/1.140 & -.006/.078/.966/1.124 \\
LD-U5 & G+RF & 0/0/0 & .004/.165/.967/1.392 & .002/.134/.972/1.279 & -.001/.114/.975/1.287 & -.003/.093/.981/1.319 \\
LD-U5 & G+SL & 0/0/0 & .002/.173/.974/1.854 & -.007/.135/.983/1.926 & -.011/.111/.985/1.976 & -.017/.086/.988/1.636 \\
LD-U5 & RB+glmnet & 0/0/0 & .001/.159/.970/1.369 & -.002/.120/.967/1.210 & -.005/.102/.968/1.141 & -.005/.077/.969/1.132 \\
LD-U5 & RB+RF & 0/0/0 & .002/.164/.968/1.397 & .001/.134/.964/1.272 & -.002/.116/.974/1.262 & -.002/.093/.981/1.327 \\
LD-U5 & RB+SL & 0/0/0 & .001/.172/.979/1.879 & -.006/.137/.985/1.884 & -.013/.112/.988/1.971 & -.016/.085/.987/1.664 \\
\addlinespace[1.2pt]
LD-U6 & G+glmnet & 0/0/0 & .019/.148/.963/1.202 & .015/.112/.960/1.082 & .015/.096/.950/1.034 & .011/.073/.962/1.068 \\
LD-U6 & G+RF & 0/0/0 & .019/.158/.965/1.239 & .017/.128/.966/1.155 & .014/.110/.970/1.197 & .012/.089/.977/1.261 \\
LD-U6 & G+SL & 0/0/0 & .017/.168/.977/1.696 & .008/.129/.982/1.822 & .006/.106/.981/1.894 & -.001/.079/.986/1.594 \\
LD-U6 & RB+glmnet & 0/0/0 & .019/.150/.963/1.188 & .015/.112/.956/1.087 & .013/.097/.949/1.030 & .011/.072/.961/1.078 \\
LD-U6 & RB+RF & 0/0/0 & .019/.157/.961/1.244 & .016/.128/.958/1.154 & .014/.112/.966/1.164 & .012/.090/.980/1.252 \\
LD-U6 & RB+SL & 0/0/0 & .016/.165/.977/1.739 & .009/.131/.986/1.795 & .004/.108/.983/1.868 & -.001/.078/.985/1.611 \\
\bottomrule
\end{longtable}
}
\end{landscape}


